CA-Stream: Attention-based pooling for interpretable image recognition

Explanations obtained from transformer-based architectures in the form of raw attention, can be seen as a class-agnostic saliency map. Additionally, attention-based pooling serves as a form of masking the in feature space. Motivated by this observation, we design an attention-based pooling mechanism intended to replace Global Average Pooling (GAP) at inference. This mechanism, called Cross-Attention Stream (CA-Stream), comprises a stream of cross attention blocks interacting with features at different network depths. CA-Stream enhances interpretability in models, while preserving recognition performance.

==> WACV_Backups/tex_wacv/abbrev.tex <==

\newcommand{\head}[1]{{\smallskip\noindent\textbf{#1}}}
\newcommand{\alert}[1]{{\color{red}{#1}}}
\newcommand{\sm}{\scriptsize}
\newcommand{\eq}[1]{(\ref{eq:#1})}

\newcommand{\Th}[1]{\textsc{#1}}
\newcommand{\mr}[2]{\multirow{#1}{*}{#2}}
\newcommand{\mc}[2]{\multicolumn{#1}{c}{#2}}
\newcommand{\tb}[1]{\textbf{#1}}
\newcommand{\ch}{\checkmark}

\newcommand{\red}[1]{{\textcolor{red}{#1}}}
\newcommand{\blue}[1]{{\textcolor{blue}{#1}}}
\newcommand{\green}[1]{{\textcolor{green}{#1}}}
\newcommand{\gray}[1]{{\textcolor{gray}{#1}}}

\newcommand{\citeme}[1]{\red{[XX]}}
\newcommand{\refme}[1]{\red{(XX)}}

\newcommand{\fig}[2][1]{\includegraphics[width=#1\linewidth]{fig/#2}}
\newcommand{\figh}[2][1]{\includegraphics[height=#1\linewidth]{fig/#2}}
\newcommand{\figa}[2][1]{\includegraphics[width=#1]{fig/#2}}
\newcommand{\figah}[2][1]{\includegraphics[height=#1]{fig/#2}}

\newcommand{\tran}{^\top}
\newcommand{\mtran}{^{-\top}}
\newcommand{\zcol}{\mathbf{0}}
\newcommand{\zrow}{\zcol\tran}

\newcommand{\ind}{\mathbbm{1}}
\newcommand{\expect}{\mathbb{E}}
\newcommand{\nat}{\mathbb{N}}
\newcommand{\zahl}{\mathbb{Z}}
\newcommand{\real}{\mathbb{R}}
\newcommand{\proj}{\mathbb{P}}
\newcommand{\prob}{\operatorname{P}}
\newcommand{\normal}{\mathcal{N}}

\newcommand{\mif}{\textrm{if}\ }
\newcommand{\other}{\textrm{otherwise}}
\newcommand{\minimize}{\textrm{minimize}\ }
\newcommand{\maximize}{\textrm{maximize}\ }
\newcommand{\st}{\textrm{subject\ to}\ }

\newcommand{\id}{\operatorname{id}}
\newcommand{\const}{\operatorname{const}}
\newcommand{\sgn}{\operatorname{sgn}}
\newcommand{\var}{\operatorname{Var}}
\newcommand{\mean}{\operatorname{mean}}
\newcommand{\trace}{\operatorname{tr}}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\vect}{\operatorname{vec}}
\newcommand{\cov}{\operatorname{cov}}
\newcommand{\sign}{\operatorname{sign}}
\newcommand{\prj}{\operatorname{proj}}

\newcommand{\softmax}{\operatorname{softmax}}
\newcommand{\clip}{\operatorname{clip}}

\newcommand{\defn}{\mathrel{:=}}
\newcommand{\peq}{\mathrel{+\!=}}
\newcommand{\meq}{\mathrel{-\!=}}

\newcommand{\paren}[1]{\left({#1}\right)}
\newcommand{\mat}[1]{\left[{#1}\right]}
\newcommand{\set}[1]{\left\{{#1}\right\}}
\newcommand{\floor}[1]{\left\lfloor{#1}\right\rfloor}
\newcommand{\ceil}[1]{\left\lceil{#1}\right\rceil}
\newcommand{\inner}[1]{\left\langle{#1}\right\rangle}
\newcommand{\norm}[1]{\left\|{#1}\right\|}
\newcommand{\abs}[1]{\left|{#1}\right|}
\newcommand{\frob}[1]{\norm{#1}_F}
\newcommand{\card}[1]{\left|{#1}\right|\xspace}

\newcommand{\diff}{\mathrm{d}}
\newcommand{\der}[3][]{\frac{\diff^{#1}#2}{\diff#3^{#1}}}
\newcommand{\ider}[3][]{\diff^{#1}#2/\diff#3^{#1}}
\newcommand{\pder}[3][]{\frac{\partial^{#1}{#2}}{\partial{{#3}^{#1}}}}
\newcommand{\ipder}[3][]{\partial^{#1}{#2}/\partial{#3^{#1}}}
\newcommand{\dder}[3]{\frac{\partial^2{#1}}{\partial{#2}\partial{#3}}}

\newcommand{\wb}[1]{\overline{#1}}
\newcommand{\wt}[1]{\widetilde{#1}}

\def\xssp{\hspace{1pt}}
\def\ssp{\hspace{3pt}}
\def\msp{\hspace{5pt}}
\def\lsp{\hspace{12pt}}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

\newcommand{\vA}{\mathbf{A}}
\newcommand{\vB}{\mathbf{B}}
\newcommand{\vC}{\mathbf{C}}
\newcommand{\vD}{\mathbf{D}}
\newcommand{\vE}{\mathbf{E}}
\newcommand{\vF}{\mathbf{F}}
\newcommand{\vG}{\mathbf{G}}
\newcommand{\vH}{\mathbf{H}}
\newcommand{\vI}{\mathbf{I}}
\newcommand{\vJ}{\mathbf{J}}
\newcommand{\vK}{\mathbf{K}}
\newcommand{\vL}{\mathbf{L}}
\newcommand{\vM}{\mathbf{M}}
\newcommand{\vN}{\mathbf{N}}
\newcommand{\vO}{\mathbf{O}}
\newcommand{\vP}{\mathbf{P}}
\newcommand{\vQ}{\mathbf{Q}}
\newcommand{\vR}{\mathbf{R}}
\newcommand{\vS}{\mathbf{S}}
\newcommand{\vT}{\mathbf{T}}
\newcommand{\vU}{\mathbf{U}}
\newcommand{\vV}{\mathbf{V}}
\newcommand{\vW}{\mathbf{W}}
\newcommand{\vX}{\mathbf{X}}
\newcommand{\vY}{\mathbf{Y}}
\newcommand{\vZ}{\mathbf{Z}}

\newcommand{\va}{\mathbf{a}}
\newcommand{\vb}{\mathbf{b}}
\newcommand{\vc}{\mathbf{c}}
\newcommand{\vd}{\mathbf{d}}
\newcommand{\ve}{\mathbf{e}}
\newcommand{\vf}{\mathbf{f}}
\newcommand{\vg}{\mathbf{g}}
\newcommand{\vh}{\mathbf{h}}
\newcommand{\vi}{\mathbf{i}}
\newcommand{\vj}{\mathbf{j}}
\newcommand{\vk}{\mathbf{k}}
\newcommand{\vl}{\mathbf{l}}
\newcommand{\vm}{\mathbf{m}}
\newcommand{\vn}{\mathbf{n}}
\newcommand{\vo}{\mathbf{o}}
\newcommand{\vp}{\mathbf{p}}
\newcommand{\vq}{\mathbf{q}}
\newcommand{\vr}{\mathbf{r}}
\newcommand{\Vs}{\mathbf{s}}
\newcommand{\vt}{\mathbf{t}}
\newcommand{\vu}{\mathbf{u}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\vw}{\mathbf{w}}
\newcommand{\vx}{\mathbf{x}}
\newcommand{\vy}{\mathbf{y}}
\newcommand{\vz}{\mathbf{z}}

\newcommand{\vone}{\mathbf{1}}
\newcommand{\vzero}{\mathbf{0}}

\newcommand{\valpha}{{\boldsymbol{\alpha}}}
\newcommand{\vbeta}{{\boldsymbol{\beta}}}
\newcommand{\vgamma}{{\boldsymbol{\gamma}}}
\newcommand{\vdelta}{{\boldsymbol{\delta}}}
\newcommand{\vepsilon}{{\boldsymbol{\epsilon}}}
\newcommand{\vzeta}{{\boldsymbol{\zeta}}}
\newcommand{\veta}{{\boldsymbol{\eta}}}
\newcommand{\vtheta}{{\boldsymbol{\theta}}}
\newcommand{\viota}{{\boldsymbol{\iota}}}
\newcommand{\vkappa}{{\boldsymbol{\kappa}}}
\newcommand{\vlambda}{{\boldsymbol{\lambda}}}
\newcommand{\vmu}{{\boldsymbol{\mu}}}
\newcommand{\vnu}{{\boldsymbol{\nu}}}
\newcommand{\vxi}{{\boldsymbol{\xi}}}
\newcommand{\vomikron}{{\boldsymbol{\omikron}}}
\newcommand{\vpi}{{\boldsymbol{\pi}}}
\newcommand{\vrho}{{\boldsymbol{\rho}}}
\newcommand{\vsigma}{{\boldsymbol{\sigma}}}
\newcommand{\vtau}{{\boldsymbol{\tau}}}
\newcommand{\vupsilon}{{\boldsymbol{\upsilon}}}
\newcommand{\vphi}{{\boldsymbol{\phi}}}
\newcommand{\vchi}{{\boldsymbol{\chi}}}
\newcommand{\vpsi}{{\boldsymbol{\psi}}}
\newcommand{\vomega}{{\boldsymbol{\omega}}}

\newcommand{\rLambda}{\mathrm{\Lambda}}
\newcommand{\rSigma}{\mathrm{\Sigma}}

\newcommand{\vLambda}{\bm{\rLambda}}
\newcommand{\vSigma}{\bm{\rSigma}}

\makeatletter
\newcommand*\bdot{\mathpalette\bdot@{.7}}
\newcommand*\bdot@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}
\makeatother

\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{cf}\onedot} \def\Cf{\emph{Cf}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot} \def\aka{a.k.a\onedot}
\def\etal{\emph{et al}\onedot}
\makeatother


==> WACV_Backups/tex_wacv/conclusion.tex <==
\section{Conclusion}

We believe we are the first to observe that attention-based pooling in transformers is the same as forming a class agnostic CAM-based saliency map and then using this map to mask the features before global average pooling, much like we mask inputs to confirm that the prediction is due to a certain object. This observation establishes that transformers have a built-in CAM-based interpretability mechanism and allows us to design a similar mechanism for convolutional networks. Masking in feature space is much more efficient than in the input space as it requires only one forward pass, although of course it is not equivalent because of interactions within the network.

Although the saliency maps obtained with our \Ours are not very different than those obtained with \gap, our approach improves a number of CAM-based interpretability methods on a number of convolutional networks according to most interpretability metrics, while preserving classification accuracy. By doing so, it also enhances the differences in performance between interpretability methods, facilitating their evaluation. Further study may be needed to improve the differentiation of saliency maps themselves, to possibly make a class specific representation more competitive and to apply the approach to more architectures, including transformers.

==> WACV_Backups/tex_wacv/defn.tex <==
% ENABLE/DISABLE COMMENTS

% \newcommand{\Col}[2]{{#2}}
% \newcommand{\Note}[2]{}
\newcommand{\Col}[2]{{\color{#1}#2}}
\newcommand{\Note}[2]{[\textbf{#1}: #2]}

\newcommand{\iavr}[1]{\Col{blue}{#1}}
\newcommand{\iavrc}[1]{\iavr{\Note{YA}{#1}}}
\newcommand{\ronan}[1]{\Col{violet}{#1}}
\newcommand{\ronanc}[1]{\ronan{\Note{RS}{#1}}}

% colors

% \definecolor{ForestGreen}{RGB}{34,139,34}
% \definecolor{Orange}{RGB}{1.0, 0.55, 0.0}
% \definecolor{Purple}{RGB}{0.58, 0.44, 0.86}
% \definecolor{LightCyan}{rgb}{0.88,1,1}
% \definecolor{TableColor}{rgb}{0.835, 0.894, 0.968}

% method
\newcommand{\relu}{{\operatorname{ReLU}}}
\newcommand{\gelu}{{\operatorname{GeLU}}}
\newcommand{\conv}{{\operatorname{conv}}}
\newcommand{\avg}{{\operatorname{avg}}}
\newcommand{\fc}{{\textsc{fc}}\xspace}
\newcommand{\gap}{{\textsc{gap}}\xspace}
\newcommand{\mlp}{{\textsc{mlp}}\xspace}
\newcommand{\ca}{{\textsc{ca}}\xspace}
\newcommand{\sa}{{\textsc{sa}}\xspace}
\newcommand{\msa}{{\textsc{msa}}\xspace}
\newcommand{\LN}{{\textsc{ln}}\xspace}
\newcommand{\cls}{{\textsc{cls}}\xspace}
\newcommand{\our}{{\textsc{ca}}}
\newcommand{\ours}{{\textsc{ca}}\xspace}
\newcommand{\Our}{{CA-Stream}}
\newcommand{\Ours}{{CA-Stream}\xspace}
\newcommand{\OURS}{{Cross Attention Stream}\xspace}
\newcommand{\PO}{{\textsc{proj}$\to$\our}\xspace}
\newcommand{\OM}{{\our$\to$\textsc{mlp}}\xspace}
\newcommand{\POM}{{\textsc{proj}$\to$\our$\to$\textsc{mlp}}\xspace}
\newcommand{\we}{\rowcolor{LightCyan}}                       % ours highlighted in table row
\newcommand{\us}[1]{{\cellcolor{LightCyan}#1}}               % ours highlighted in table cell
\newcommand{\all}{\tikz{\draw[white,fill=black,line width=0.4pt] (0,0) circle (1.2pt);}}

% experiments
\newcommand{\imagenet}{{ImageNet-1k}\xspace}
%\newcommand{\resnet}{{ResNet-$18$}\xspace}
%\newcommand{\resnet50}{{ResNet-$50$}\xspace}
%\newcommand{\vits}{{ViT-S}\xspace}
%\newcommand{\vitt}{{ViT-T}\xspace}
%\newcommand{\convnexts}{{ConvNeXT-S}\xspace}
%\newcommand{\cifar10}{CIFAR-$10$\xspace}
%\newcommand{\cifar100}{CIFAR-$100$\xspace}
%\newcommand{\flowers}{Oxford Flowers\xspace}
%\newcommand{\cub}{CUB-$200$\xspace}
%\newcommand{\voc12}{VOC$12$\xspace}
%\newcommand{\voc7}{VOC$07$\xspace}
%\newcommand{\coco}{COCO\xspace}

\newcommand{\gain}[1]{}
\newcommand{\gp}[1]{{\color{ForestGreen}#1}}
\newcommand{\gn}[1]{\red{#1}}
\newcommand{\se}[1]{\blue{#1}}
\newcommand{\sota}[1]{\red{\textbf{#1}}}
\newcommand{\negative}[1]{\blue{#1}}

\definecolor{TableColor}{rgb}{0.835, 0.894, 0.968}

==> WACV_Backups/tex_wacv/exp_ablation-1.tex <==
    \subsection{Ablation}
    \label{sec:gen_ablation}
    To make sense of our approach, we conduct ablation experiments on interpretable recognition tasks. For these experiments, we opt to experiment on ResNet50 because of its modularity and ease of modification. First, we demonstrate the differences between the possible variations of the CA-Block, then we experiment with the placement of said  mechanism on a given backbone alongside its effects on interpretability, continuing with an study of the interpretability capabilities of the attention branch, to finish, we remonstrate a comparison between our chosen approach when training from  pretrained weights and scratch.

    \paragraph{Cross Attention block proposals}
    Following the proposals for the CA block found on \autoref{subsec:variations}, we compare the effect on accuracy when adding one of them to the backbone (just after the last residual block). \autoref{tab:CA_variations} demonstrates this assessment.
    
    \begin{table}[H]
        \centering
        %\resizebox{\columnwidth}{!}{%
        \scriptsize
        %\resizebox{5.5cm}{!}{%
        %\resizebox{\columnwidth}{!}{%}
        \begin{tabular}{lcc}\\\toprule
             \Th{Block Type}&\Th{$\#$Params}&\Th{Acc}\\\midrule
             CA&4.20M&74.63\\
             Proj$\rightarrow$CA&12.58M&74.19\\
             CA$\rightarrow$MLP&20.97M&-\\
             Proj$\rightarrow$CA$\rightarrow$MLP&29.36M&-\\\bottomrule
        \end{tabular}
        %}
        \caption{Comparison of classification performance when one cross attention block is added into the last residual block of ResNet-50.}
        \label{tab:CA_variations}
    \end{table}
    %To start with the proposals for the CA-block,
    We observe that the introduction of the basic design of the cross attention module outperforms the classification properties of that which uses projection of the input features to compute the subsequent representation. We hypothesize that maintaining the features without any projection allows the [class] token to better collect global information, as patch information is maintained in the same space that the already trained classifier relies on to perform classification. 
    On another hand, we also note that the introduction of an MLP to update said representation is not feasible given instability during training, for this reason we decide not to pursue further experimentation with this idea.
    %We observe that there is a notable difference in performance between the adoption of the basic block and that which has projections for the features that are used to compute the subsequent representation. However, we hypothesize that this difference is due in large manner because of the parameter overhead for the feature projection. Moreover, we also note that introducing an MLP to update the representation computed in the attention mechanism is not possible given instability during training, for this reason we consider that further experimentation with this variant is not desired given the nature of the idea.% towards providing a lightweight manner to produce interpretable recognition.
    \begin{table}[H]
        \centering
        \scriptsize
        %\resizebox{5.5cm}{!}{%
        %\resizebox{\columnwidth}{!}{%}
        \begin{tabular}{lcc}\toprule
             \Th{Block Type}&\Th{$\#$Params}&\Th{Accuracy}\\\midrule
             CA&6.96M&74.70\\
             Proj$\rightarrow$CA&18.13M&74.41\\\bottomrule
        \end{tabular}
        %}
        \caption{Comparisson of classification performance for CLS-Streams using different CA block designs using ResNet-50 as backbone}
        \label{tab:dif_streams}
    \end{table}
    %Moving on, we experiment with the inclusion of a stream of CA blocks alongside the backbone. For this, we place a block whenever we increase the dimensionality of features at different residual blocks. As noted on Table \ref{tab:dif_streams}, we observe that while a single CA block with feature projections performs better than one without them, however, the aggregation of multiple basic CA blocks produces better results than the aforementioned proposal, while also reducing the amount of trainable parameters. In the spirit of providing explanations in a simple and straightforward manner, we conduct our experimentation with the basic CA design.
    % On another hand, we point the sharp contrast in the parameter count when we add more operations to this mechanism,  it is combining this observation with the idea of providing explanations for a given model in a straightforward manner, that we opt to build the CLS-Stream on the simplest manner possible. For this reason, for the rest of the paper we choose this version by default.
    Moving on, we experiment with the CLS-Stream using either CA-block proposal. As noted on \autoref{tab:dif_streams}, we observe that the stream made of basic CA blocks performs better than that which uses projections for the attention mechanism. Moreover, we observe that this aggregation of CA blocks remains lightweight and overall improves the performance for the aforementioned block design. On top of this, we also note that most of the computation weight lies within the last residual stages, as it depends directly on the channel dimension which is largest in these depths. In the spirit of providing explanations in a simple and straightforward manner, we conduct our experimentation with the basic CA design.


    %% Under revision from here
    \paragraph{CLS-Stream design}
    \label{ab:placement}
    %To assess the effect of the placement of the CA blocks, we conduct experiments across the width the model, varying the starting point for this approach; departing from the first residual block onto the last residual block. For this family of experiments we evaluate accuracy and interpretability metrics (reported on tables \ref{tab:acc_tab} and \ref{tab:intrecog-resnet}) , as it is in our best interest to obtain a model that preserves if not improves the classification performance, while providing enhanced explanations.
    To validate the design of the CLS-Stream, we conduct experiments across the depth the model; varying the starting point for this approach: departing from the first residual stage onto the last residual one. For this family of experiments we evaluate accuracy and interpretability metrics reported on \autoref{tab:intrecog-resnet}, as it is in our best interest to obtain a model that preserves if not improves the classification performance, while providing enhanced explanations.
    % \begin{table}[H]
    %     \centering

    %     \caption{Classification metrics for ResNet-50 with different CLS stream propositions.}
    %     \label{tab:acc_tab}
    % \end{table}
    %Regarding classification performance, we report the CA module placements, the CLS token starting dimension and the total parameter count and accuracy values.
    \textbf{Check}
    %We observe that there is a stark difference between on accuracy when comparing a CLS stream made up of multiple CA blocks, and one composed of solely one; this difference is clearer when we compare the two simplest CLS streams, (R$_3\rightarrow\mbox{R}_4$) and (R$_4$). We hypothesize that one possible explanation for these discrepancies lies within the complexity of training the CLS token and the amount of interactions that it can have with the features flowing from the backbone. Following this, we observe that having a deeper stream allows for a smaller classification token to be learnt, as by design its dimensions are projected to those in the following stages in the backbone to support attention computation.  We argue that the more communication with features, the more CLS can learn, alongside its projections. %We argue that this contrast in performance takes into consideration more interactions between the CLS token %it is important to note that the increment in trainable parameters is found alongside the depth of the network. We observe that the layers that present a larger quantity of parameters are found out closer to the classifier

    % Following the focus on interpretability evaluation, we generate saliency maps for each of the aforementioned models and we evaluate them on terms of AD, AG, IC, Ins and Del. Results are reported on Table \ref{tab:intrecog-resnet}
    \begin{table}[t]
        \centering
        \scriptsize
        \setlength{\tabcolsep}{2.5pt}
        %\resizebox{\columnwidth}{!}{%}
        \begin{tabular}{cccccc}\toprule
             Placement&CLS Dimension&\#Params&Accuracy\\\midrule
             $\mbox{R}_0\rightarrow\mbox{R}_4$&$1\times64$&6.963.264&\textbf{74.70}\\
             $\mbox{R}_1\rightarrow\mbox{R}_4$&$1\times256$&6.947.072&74.67\\
             $\mbox{R}_2\rightarrow\mbox{R}_4$&$1\times512$&6.816.256&74.67\\
             $\mbox{R}_3\rightarrow\mbox{R}_4$&$1\times1024$&6.292.480&74.67\\
             $\mbox{R}_4\rightarrow\mbox{R}_4$&$1\times2048$&4.196.352&74.63\\\bottomrule
        \end{tabular}
        %}
        
        \bigskip
        %\resizebox{\columnwidth}{!}{%
        \begin{tabular}{llccccc}\toprule
            \Th{Method}&\Th{Placement}&\Th{AD$\downarrow$}&\Th{AG$\uparrow$}&\Th{AI$\uparrow$}&\Th{I$\uparrow$}&\Th{D$\downarrow$}\\\midrule
            \mr{5}{\Th{Grad-CAM}}&$\mbox{R}_0-\mbox{R}_4$&\textbf{12.54}&\blue{22.67}&\blue{48.56}&75.53&13.50\\ % Checked
             &$\mbox{R}_1-\mbox{R}_4$&12.69&22.65&48.31&75.53&13.41\\ % Checked
             &$\mbox{R}_2-\mbox{R}_4$&\textbf{12.54}&21.67&\textbf{48.58}&75.54&13.50\\ % Running
             &$\mbox{R}_3-\mbox{R}_4$&12.69&22.28&47.89&\blue{75.55}&\textbf{13.40}\\ % Running
             &$\mbox{R}_4-\mbox{R}_4$&12.77&20.65&47.14&74.32&13.37\\\hline % Checked
            \mr{5}{\Th{Grad-CAM++}}&$\mbox{R}_0-\mbox{R}_4$&13.99&19.29&\blue{44.60}&75.21&13.78\\ % Checked
             &$\mbox{R}_1-\mbox{R}_4$&13.99&19.29&\textbf{44.62}&75.21&13.78\\ % Checked
             &$\mbox{R}_2-\mbox{R}_4$&\blue{13.71}&\blue{19.90}&45.43&75.34&\blue{13.50}\\ % Running
             &$\mbox{R}_3-\mbox{R}_4$&\textbf{13.69}&19.61&45.04&\blue{75.36}&\blue{13.50}\\ % Running
             &$\mbox{R}_4-\mbox{R}_4$&13.67&18.36&44.40&Check&Check\\\hline % Checked
            \mr{5}{\Th{Score-CAM}}&$\mbox{R}_0-\mbox{R}_4$&\blue{7.09}&23.65&54.20&74.91&14.68\\ % Checked
             &$\mbox{R}_1-\mbox{R}_4$&\blue{7.09}&23.65&54.20&\blue{74.92}&14.68\\ % Checked
             &$\mbox{R}_2-\mbox{R}_4$&\blue{7.09}&\blue{23.66}&54.21&74.91&14.68\\ % Running
             &$\mbox{R}_3-\mbox{R}_4$&7.74&23.03&\blue{52.92}&\textbf{74.97}&\blue{14.65}\\ % Running
             &$\mbox{R}_4-\mbox{R}_4$&Check&Check&Check&Check&Check\\\bottomrule % Checked
        \end{tabular}
       % }
        \caption{\emph{Recognition metrics for ResNet-50 and CLS stream design.} \textbf{Top} Stream design and classification metrics. \textbf{Bottom} Interpretable Recognition Metrics with the addition of the CLS stream across different stages of the network.}% We report the interpretable recognition metrics obtained by varying placement of the CLS stream from the first to the last residual blocks it receives features from.}
        \label{tab:intrecog-resnet}
    \end{table}

    % To begin with, we observe that 
    From the different class activation mappings interpretability results, we observe that the stream configuration that interacts the most with the backbone obtains the best metrics overall, taking into consideration the classification performance. On another hand, we take special notice on the performance when using the lightest stream of only one CA block. We note that its interpretable properties present a sharp contrast when compared to those of different approaches, presenting remarkable improvements in terms of AG, Ins and Del; and notable losses in terms of AD and AI. We place special consideration on the results obtained for Score-CAM, as for it the difference in performance increases for all methods when compared to CA on R$_4$ alone.%; having improvements of 3, 16 and 6 points for AD, AG, AI respectively.
    % Until here
    \paragraph{Class Agnostic CLS}
    As mentioned on \autoref{subsec:motiv}, we observed that while there is a difference between CAM-based saliency maps ~\eq{sal} and attention ~\eq{connection}, it is possible to extend ~\eq{connection} using a query vector per class, making it class specific. For this goal, during training we forward the weight vector relating to the groundtruth class for a given image, and during inference we forward the weight vector related to the predicted class by the backbone. This way, during training we update the [class] tokens according to the groundtruth labels in the minibatch.

    \begin{table}[H]
        \centering
        \scriptsize
        \setlength{\tabcolsep}{2.5pt}
        %\resizebox{\columnwidth}{!}{%
        \begin{tabular}{lllccccc}\toprule                    
            Repr&Accuracy&Method&AD$\downarrow$&AG$\uparrow$&AI$\uparrow$&I$\uparrow$&D$\downarrow$\\\midrule
            % \multirow{3}{*}{GAP}&\multirow{3}{*}{74.55}&Grad-CAM&13.04&17.56&44.47&72.57&13.24\\
            %  & &Grad-CAM++&13.79&15.87&42.08&72.32&13.33\\
            %  & &Score-CAM&13.64&12.98&44.53&62.56&11.37\\\hline %
            \multirow{3}{*}{CLS$_T$}&\multirow{3}{*}{74.70}&Grad-CAM&12.54&22.67&48.56&75.53&13.50\\
             & &Grad-CAM++&13.99&19.29&44.60&75.21&13.78\\
             & &Score-CAM&7.09&23.65&54.20&74.91&14.68\\\midrule
             \multirow{3}{*}{CLS$_M$}&\multirow{3}{*}{74.68}&Grad-CAM&12.53&22.66&48.58&75.54&13.50\\
             & &Grad-CAM++&13.99&19.28&44.62&75.20&13.78\\
             & &Score-CAM&TBA&TBA&TBA&TBA&TBA\\\bottomrule
        \end{tabular}
        %}
        \caption{Interpretable recognition comparison between Class agnostic tokens (\emph{CLS$_T$}) and Class specific tokens (\emph{CLS$_M$}).}
        \label{tab:TokenvMatrix}

    \end{table}

    \autoref{tab:TokenvMatrix} presents a comparison of the CLS-Stream using class agnostic and class specific representations. We observe that presenting a class dependent representation for the CLS Stream to learn, provides no remarkable diferences when compared with the standard class agnostic representation. Similar to \cite{touvron2021augmenting} our class dependent representation is capable of providing independent class maps, however to do so we do not require any fine-tuning whatsoever. 
    % For these reasons and in hopes of maintaining a simple approach

    \paragraph{Stream Attention Interpretability}
    Based on equation \ref{eq:connection} and inspired by \cite{abnar2020quantifying}, we note that we can visualize the flow of information across the CLS-Stream for every CA block. Nevertheless, from the aforementioned work, we find that Attention Rollout is not so desired given complications in its calculation. On \autoref{fig:compmethods} we observe some differences between Attention and different CAM proposals. % Define Attention
    % With this in mind we first demonstrate the similarities between Grad-CAM and Raw Attention in Figure \ref{fig:rawatt_gradcam}.
    % Conversely, following the similarity between CAM methods and attention, we observe that attention can be used to compute saliency maps. We present the similarities for these kinds of visualizations in figure \ref{fig:rawatt_gradcam}

    % \begin{figure}[H]
    %     \centering
    %     % \resizebox{\columnwidth}{!}{%
    %     \begin{tabular}{cccc}
    %         {}&Input Image & Grad-CAM & Raw Attention\\
    %         % {\rotatebox{90}{classname}}&{\includegraphics[width=0.15\textwidth]{}}&{\includegraphics[width=0.15\textwidth]{}}&{\includegraphics[width=0.15\textwidth]{}}\\
    %         % {\rotatebox{90}{classname}}&{\includegraphics[width=0.15\textwidth]{}}&{\includegraphics[width=0.15\textwidth]{}}&{\includegraphics[width=0.15\textwidth]{}}\\
    %         % {\rotatebox{90}{classname}}&{\includegraphics[width=0.15\textwidth]{}}&{\includegraphics[width=0.15\textwidth]{}}&{\includegraphics[width=0.15\textwidth]{}}\\
    %     \end{tabular}
    %     % }
    %     \caption{Visual comparison between Grad-CAM and Raw Attention}
    %     \label{fig:rawatt_gradcam}
    % \end{figure}

    Moving on, we evaluate these attention maps following the approach for interpretable recognition. As noted on \autoref{tab:rawatt_gradcam}, raw attention presents a similar if not a bit worse performance in comparison to Grad-CAM. It could be argued that according to the similarities between CAM based approaches and attention ones described in ~\eq{connection}, a direct comparison is plausible; although not proper, knowing that raw attention uses softmax as non-linearity.

    \begin{table}[H]
        \centering
        \scriptsize
        %\resizebox{\columnwidth}{!}{%}
        \begin{tabular}{lccccc}\toprule
             \Th{Method}&\Th{AD}$\downarrow$&\Th{AG$\uparrow$}&\Th{AI$\uparrow$}&\Th{I$\uparrow$}&\Th{D$\downarrow$}\\\midrule
             Raw-Attention&13.42&15.76&41.48&73.86&16.29\\
             Grad-CAM&12.54&22.67&48.56&75.53&13.50\\\bottomrule
        \end{tabular}
        %}
        \caption{Comparison of interpretable performance between Raw Attention and Grad-CAM}
        \label{tab:rawatt_gradcam}
    \end{table}

    % Can be deleted if so
    \paragraph{Training from Scratch}
    % Rephrasing to make emph on post-hoc and argue that while it is possible, acc is not dropped too much. It's more interesting to do post-hoc (...) sic.
    % Other comparisons, SCOUTER. Maybe play with Conformer

    One of the latest observations from our approach answers to the question \textit{what would happen if we trained each model from scratch?}. Following existing training regime for ResNet50, we begin by training a baseline model which will be a replica of that found off the shelf; we make use of this model as a control further down the experimentation. Then we train a model with the CLS stream in a similar fashion. We present the evolution of the training error in \autoref{fig:scratch_freeze}

    \begin{figure}[H]
        \centering
            \begin{tikzpicture}
                \begin{axis}[width=\columnwidth,height=2in, no markers, xlabel=epoch, ylabel=error,
                            grid=both, grid style={line width=.1pt, draw=gray!10}, major grid style={line width=.2pt,draw=gray!50},]
                    [xlabel = epochs,
                    ylabel = top1 err]
                    \addplot table [x=epoch, y=top1err, col sep=comma, mark=none] {Data/r50base_scratch.csv};
                    \addplot table [x=epoch, y=top1err, col sep=comma, mark=none] {Data/r50stream_scratch.csv};
                    \addplot table [x=epoch, y=top1err, col sep=comma, mark=none] {Data/r50stream_shelf.csv};
                    \legend{Backbone,
                            Backbone+Stream,
                            Stream}
                \end{axis}
             \end{tikzpicture}
        \label{fig:scratch_freeze}
        \caption{Curves of training procedure on ImageNet-1k for ResNet50 for the baseline model (blue) vs baseline and CLS-stream (red) and just training the stream. We show the top-1 training error for the different approaches.}
    \end{figure}

    Moreover, these differences are better quantified with the \textbf{(WIP)}

    %% Top design, bottom interp metrics
    %% More parts for experiments

    % Ablation of histogram of diferences with extreme cases

==> WACV_Backups/tex_wacv/exp_ablation-2.tex <==
\subsection{Ablation}
\label{sec:gen_ablation}

To make sense of our approach, we conduct ablation experiments on interpretable recognition tasks. For these experiments, we opt to experiment on ResNet50 because of its modularity and ease of modification. First, we demonstrate the differences between the possible variations of the CA-Block, then we experiment with the placement of said  mechanism on a given backbone alongside its effects on interpretability, continuing with an study of the interpretability capabilities of the attention branch, to finish, we remonstrate a comparison between our chosen approach when training from  pretrained weights and scratch.

%------------------------------------------------------------------------------

\paragraph{Cross attention block design}

Following transformers~\cite{NIPS2017_3f5ee243,dosovitskiy2020image}, it is possible to add more layers in the cross attention block. We consider two variants. One, referred to as \PO, uses linear projections $W_\ell^K, W_\ell^V \in \real^{d_\ell \times d_\ell}$ on the key and value
\begin{equation}
	\ca_\ell(\vq_\ell, F_\ell) \defn (F_\ell W^V_\ell)\tran h_\ell(F_\ell W^K_\ell \vq_\ell)\in \real^{d_\ell}.
\label{eq:proj_ca}
\end{equation}
In another variant, referred to as \OM, an MLP follows each cross attention block, defined as
\begin{equation}
	\mlp_\ell(\vq_\ell) = W_\ell^2 \gelu(W_\ell^1 \vq_\ell + b_\ell^1) + b_\ell^2,
\label{eq:mlp_ca}
\end{equation}
where $W_\ell^1 \in \real^{2d_\ell \times d_\ell}$ and $W_\ell^1 \in \real^{d_\ell \times 2d_\ell}$. In both cases, equation~\eq{qk-layer} remains. The combination of the two variants is referred to as \POM.


We compare the effect on accuracy when adding one of the variants to the backbone (just after the last residual block). \autoref{tab:CA_variations} demonstrates this assessment.

%------------------------------------------------------------------------------
\begin{table}
\centering
%\resizebox{\columnwidth}{!}{%
\scriptsize
\begin{tabular}{lcc}\\\toprule
	\Th{Block Type}&\Th{$\#$Params}&\Th{Acc}\\\midrule
	CA&4.20M&74.63\\
	Proj$\rightarrow$CA&12.58M&74.19\\
	CA$\rightarrow$MLP&20.97M&-\\
	Proj$\rightarrow$CA$\rightarrow$MLP&29.36M&-\\\bottomrule
\end{tabular}
%}
\vspace{3pt}
\caption{Comparison of classification performance when one cross attention block is added into the last residual block of ResNet-50.}
\label{tab:CA_variations}
\end{table}
%------------------------------------------------------------------------------

We observe that the introduction of the basic design of the cross attention module outperforms the classification properties of that which uses projection of the input features to compute the subsequent representation. We hypothesize that maintaining the features without any projection allows the [class] token to better collect global information, as patch information is maintained in the same space that the already trained classifier relies on to perform classification. 
On another hand, we also note that the introduction of an MLP to update said representation is not feasible given instability during training, for this reason we decide not to pursue further experimentation with this idea.
%We observe that there is a notable difference in performance between the adoption of the basic block and that which has projections for the features that are used to compute the subsequent representation. However, we hypothesize that this difference is due in large manner because of the parameter overhead for the feature projection. Moreover, we also note that introducing an MLP to update the representation computed in the attention mechanism is not possible given instability during training, for this reason we consider that further experimentation with this variant is not desired given the nature of the idea.% towards providing a lightweight manner to produce interpretable recognition.

%------------------------------------------------------------------------------
\begin{table}
\centering
\scriptsize
%\resizebox{\columnwidth}{!}{%}
\begin{tabular}{lcc}\toprule
	\Th{Block Type}&\Th{$\#$Params}&\Th{Accuracy}\\\midrule
	CA&6.96M&74.70\\
	Proj$\rightarrow$CA&18.13M&74.41\\\bottomrule
\end{tabular}
%}
\vspace{3pt}
\caption{Comparison of classification performance for CLS-Streams using different CA block designs using ResNet-50 as backbone}
\label{tab:dif_streams}
\end{table}
%------------------------------------------------------------------------------

%Moving on, we experiment with the inclusion of a stream of CA blocks alongside the backbone. For this, we place a block whenever we increase the dimensionality of features at different residual blocks. As noted on Table \ref{tab:dif_streams}, we observe that while a single CA block with feature projections performs better than one without them, however, the aggregation of multiple basic CA blocks produces better results than the aforementioned proposal, while also reducing the amount of trainable parameters. In the spirit of providing explanations in a simple and straightforward manner, we conduct our experimentation with the basic CA design.
% On another hand, we point the sharp contrast in the parameter count when we add more operations to this mechanism,  it is combining this observation with the idea of providing explanations for a given model in a straightforward manner, that we opt to build the CLS-Stream on the simplest manner possible. For this reason, for the rest of the paper we choose this version by default.
Moving on, we experiment with the CLS-Stream using either CA-block proposal. As noted on \autoref{tab:dif_streams}, we observe that the stream made of basic CA blocks performs better than that which uses projections for the attention mechanism. Moreover, we observe that this aggregation of CA blocks remains lightweight and overall improves the performance for the aforementioned block design. On top of this, we also note that most of the computation weight lies within the last residual stages, as it depends directly on the channel dimension which is largest in these depths. In the spirit of providing explanations in a simple and straightforward manner, we conduct our experimentation with the basic CA design.

%------------------------------------------------------------------------------

\paragraph{\Ours placement}
\label{ab:placement}

To validate the design of \Ours, we measure the effect of its depth on its performance \vs the baseline \gap in terms of both classification accuracy / number of parameters and classification metrics for interpretability. In particular, we place the stream in parallel to the network $f$, starting at stage $\ell$ and running through stage $L$, the last stage of $f$, where $0 \le \ell \le L$. Results are reported in \autoref{tab:intrecog-resnet}.

\textbf{Check}

%------------------------------------------------------------------------------
\begin{table}
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
%\resizebox{\columnwidth}{!}{%}
\begin{tabular}{lcccccc}\toprule
	\mc{7}{\Th{Accuracy and Parameters}}\\\midrule
	&\Th{Placement}&\mc{2}{\Th{CLS dim}}&\mc{2}{\Th{\#Param}}&\Th{Acc}\\\midrule
	
	&$S_0-S_4$&\mc{2}{$64$}  &\mc{2}{6.96M}&\textbf{74.70}\\  % 6.963.264
	&$S_1-S_4$&\mc{2}{$256$} &\mc{2}{6.95M}&74.67\\           % 6.947.072
	&$S_2-S_4$&\mc{2}{$512$} &\mc{2}{6.82M}&74.67\\           % 6.816.256
	&$S_3-S_4$&\mc{2}{$1024$}&\mc{2}{6.29M}&74.67\\           % 6.292.480
	&$S_4-S_4$&\mc{2}{$2048$}&\mc{2}{4.20M}&74.63\\\midrule   % 4.196.352
	
	\mc{7}{\Th{Interpretability Metrics}}\\\midrule
	\Th{Method}&\Th{Placement}&\Th{AD$\downarrow$}&\Th{AG$\uparrow$}&\Th{AI$\uparrow$}&\Th{I$\uparrow$}&\Th{D$\downarrow$}\\\midrule
	
	\mr{5}{\Th{Grad-CAM}}&$S_0-S_4$&\textbf{12.54}&\blue{22.67}&\blue{48.56}&75.53&13.50\\ % Checked
		&$S_1-S_4$&12.69&22.65&48.31&75.53&13.41\\ % Checked
		&$S_2-S_4$&\textbf{12.54}&21.67&\textbf{48.58}&75.54&13.50\\ % Running
		&$S_3-S_4$&12.69&22.28&47.89&\blue{75.55}&\textbf{13.40}\\ % Running
		&$S_4-S_4$&12.77&20.65&47.14&74.32&13.37\\\midrule % Checked
		
	\mr{5}{\Th{Grad-CAM++}}&$S_0-S_4$&13.99&19.29&\blue{44.60}&75.21&13.78\\ % Checked
		&$S_1-S_4$&13.99&19.29&\textbf{44.62}&75.21&13.78\\ % Checked
		&$S_2-S_4$&\blue{13.71}&\blue{19.90}&45.43&75.34&\blue{13.50}\\ % Running
		&$S_3-S_4$&\textbf{13.69}&19.61&45.04&\blue{75.36}&\blue{13.50}\\ % Running
		&$S_4-S_4$&13.67&18.36&44.40&74.190&13.30\\\midrule % Checked
		
	\mr{5}{\Th{Score-CAM}}&$S_0-S_4$&\blue{7.09}&23.65&54.20&74.91&14.68\\ % Checked
		&$S_1-S_4$&\blue{7.09}&23.65&54.20&\blue{74.92}&14.68\\ % Checked
		&$S_2-S_4$&\blue{7.09}&\blue{23.66}&54.21&74.91&14.68\\ % Running
		&$S_3-S_4$&7.74&23.03&\blue{52.92}&\textbf{74.97}&\blue{14.65}\\ % Running
		&$S_4-S_4$&Check&Check&Check&Check&Check\\\bottomrule % Checked
\end{tabular}
% }
\vspace{3pt}
\caption{\emph{Effect of stream placement} on accuracy, parameters and interpretability metrics of \Ours \vs baseline \gap for ResNet-50 and different interpretability methods on ImageNet. $S_\ell-S_L$: \Ours runs from stage $\ell$ to $L$ (last); \Th{$\#$Param}: parameter or \Ours only; Bold: best per method per metric.}
\label{tab:intrecog-resnet}
\end{table}
%------------------------------------------------------------------------------

From the different class activation mappings interpretability results, we observe that the stream configuration that interacts the most with the backbone obtains the best metrics overall, taking into consideration the classification performance. On another hand, we take special notice on the performance when using the lightest stream of only one CA block. We note that its interpretable properties present a sharp contrast when compared to those of different approaches, presenting remarkable improvements in terms of AG, Ins and Del; and notable losses in terms of AD and AI. We place special consideration on the results obtained for Score-CAM, as for it the difference in performance increases for all methods when compared to CA on R$_4$ alone.%; having improvements of 3, 16 and 6 points for AD, AG, AI respectively.

%------------------------------------------------------------------------------

\paragraph{Class-agnostic CLS}

As mentioned on \autoref{subsec:motiv}, we observed that while there is a difference between CAM-based saliency maps ~\eq{sal} and attention ~\eq{connection}, it is possible to extend ~\eq{connection} using a query vector per class, making it class specific. For this goal, during training we forward the weight vector relating to the groundtruth class for a given image, and during inference we forward the weight vector related to the predicted class by the backbone. This way, during training we update the [class] tokens according to the groundtruth labels in the minibatch.

%------------------------------------------------------------------------------
\begin{table}
\centering
\scriptsize
\setlength{\tabcolsep}{2.5pt}
%\resizebox{\columnwidth}{!}{%
\begin{tabular}{lllccccc}\toprule                    
	Repr&Accuracy&Method&AD$\downarrow$&AG$\uparrow$&AI$\uparrow$&I$\uparrow$&D$\downarrow$\\\midrule
	% \multirow{3}{*}{GAP}&\multirow{3}{*}{74.55}&Grad-CAM&13.04&17.56&44.47&72.57&13.24\\
	%  & &Grad-CAM++&13.79&15.87&42.08&72.32&13.33\\
	%  & &Score-CAM&13.64&12.98&44.53&62.56&11.37\\\hline %
	\multirow{3}{*}{CLS$_T$}&\multirow{3}{*}{74.70}&Grad-CAM&12.54&22.67&48.56&75.53&13.50\\
		& &Grad-CAM++&13.99&19.29&44.60&75.21&13.78\\
		& &Score-CAM&7.09&23.65&54.20&74.91&14.68\\\midrule
		\multirow{3}{*}{CLS$_M$}&\multirow{3}{*}{74.68}&Grad-CAM&12.53&22.66&48.58&75.54&13.50\\
		& &Grad-CAM++&13.99&19.28&44.62&75.20&13.78\\
		& &Score-CAM&TBA&TBA&TBA&TBA&TBA\\\bottomrule
\end{tabular}
%}
\vspace{3pt}
\caption{Interpretable recognition comparison between Class agnostic tokens (\emph{CLS$_T$}) and Class specific tokens (\emph{CLS$_M$}).}
\label{tab:TokenvMatrix}
\end{table}
%------------------------------------------------------------------------------

\autoref{tab:TokenvMatrix} presents a comparison of the CLS-Stream using class agnostic and class specific representations. We observe that presenting a class dependent representation for the CLS Stream to learn, provides no remarkable diferences when compared with the standard class agnostic representation. Similar to \cite{touvron2021augmenting} our class dependent representation is capable of providing independent class maps, however to do so we do not require any fine-tuning whatsoever. 
% For these reasons and in hopes of maintaining a simple approach

%------------------------------------------------------------------------------

\paragraph{Stream attention interpretability}

Based on equation \ref{eq:connection} and inspired by \cite{abnar2020quantifying}, we note that we can visualize the flow of information across the CLS-Stream for every CA block. Nevertheless, from the aforementioned work, we find that Attention Rollout is not so desired given complications in its calculation. On \autoref{fig:compmethods} we observe some differences between Attention and different CAM proposals. % Define Attention
% With this in mind we first demonstrate the similarities between Grad-CAM and Raw Attention in Figure \ref{fig:rawatt_gradcam}.
% Conversely, following the similarity between CAM methods and attention, we observe that attention can be used to compute saliency maps. We present the similarities for these kinds of visualizations in figure \ref{fig:rawatt_gradcam}

% \begin{figure}[H]
%     \centering
%     % \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{cccc}
%         {}&Input Image & Grad-CAM & Raw Attention\\
%         % {\rotatebox{90}{classname}}&{\includegraphics[width=0.15\textwidth]{}}&{\includegraphics[width=0.15\textwidth]{}}&{\includegraphics[width=0.15\textwidth]{}}\\
%         % {\rotatebox{90}{classname}}&{\includegraphics[width=0.15\textwidth]{}}&{\includegraphics[width=0.15\textwidth]{}}&{\includegraphics[width=0.15\textwidth]{}}\\
%         % {\rotatebox{90}{classname}}&{\includegraphics[width=0.15\textwidth]{}}&{\includegraphics[width=0.15\textwidth]{}}&{\includegraphics[width=0.15\textwidth]{}}\\
%     \end{tabular}
%     % }
%     \caption{Visual comparison between Grad-CAM and Raw Attention}
%     \label{fig:rawatt_gradcam}
% \end{figure}

Moving on, we evaluate these attention maps following the approach for interpretable recognition. As noted on \autoref{tab:rawatt_gradcam}, raw attention presents a similar if not a bit worse performance in comparison to Grad-CAM. It could be argued that according to the similarities between CAM based approaches and attention ones described in ~\eq{connection}, a direct comparison is plausible; although not proper, knowing that raw attention uses softmax as non-linearity.

%------------------------------------------------------------------------------
\begin{table}
\centering
\scriptsize
%\resizebox{\columnwidth}{!}{%}
\begin{tabular}{lccccc}\toprule
		\Th{Method}&\Th{AD}$\downarrow$&\Th{AG$\uparrow$}&\Th{AI$\uparrow$}&\Th{I$\uparrow$}&\Th{D$\downarrow$}\\\midrule
		Raw-Attention&13.42&15.76&41.48&73.86&16.29\\
		Grad-CAM&12.54&22.67&48.56&75.53&13.50\\\bottomrule
\end{tabular}
%}
\vspace{3pt}
\caption{Comparison of interpretable performance between Raw Attention and Grad-CAM}
\label{tab:rawatt_gradcam}
\end{table}
%------------------------------------------------------------------------------


%% Top design, bottom interp metrics
%% More parts for experiments

% Ablation of histogram of diferences with extreme cases


==> WACV_Backups/tex_wacv/exp_ablation.tex <==
\subsection{Ablation}
\label{sec:gen_ablation}

We conduct ablation experiments on ResNet50 because of its modularity and ease of modification. We investigate the effect of the cross attention block design, the placement of the \Ours relative to the backbone network.
The appendix further includes an extra experiments regarding class agnostic \vs class specific representations.

%------------------------------------------------------------------------------

\paragraph{Cross attention block design}

Following transformers~\cite{NIPS2017_3f5ee243,dosovitskiy2020image}, it is possible to add more layers in the cross attention block. We consider a variant referred to as \PO, which uses linear projections $W_\ell^K, W_\ell^V \in \real^{d_\ell \times d_\ell}$ on the key and value
\begin{equation}
	\ca_\ell(\vq_\ell, F_\ell) \defn (F_\ell W^V_\ell)\tran h_\ell(F_\ell W^K_\ell \vq_\ell)\in \real^{d_\ell},
\label{eq:proj_ca}
\end{equation}
while equation~\eq{qk-layer} remains.

% We consider two variants. One, referred to as \PO, uses linear projections $W_\ell^K, W_\ell^V \in \real^{d_\ell \times d_\ell}$ on the key and value
% \begin{equation}
% 	\ca_\ell(\vq_\ell, F_\ell) \defn (F_\ell W^V_\ell)\tran h_\ell(F_\ell W^K_\ell \vq_\ell)\in \real^{d_\ell}.
% \label{eq:proj_ca}
% \end{equation}
% In another variant, referred to as \OM, an MLP follows each cross attention block, defined as
% \begin{equation}
% 	\mlp_\ell(\vq_\ell) = W_\ell^2 \gelu(W_\ell^1 \vq_\ell + b_\ell^1) + b_\ell^2,
% \label{eq:mlp_ca}
% \end{equation}
% where $W_\ell^1 \in \real^{2d_\ell \times d_\ell}$ and $W_\ell^1 \in \real^{d_\ell \times 2d_\ell}$. In both cases, equation~\eq{qk-layer} remains. The combination of the two variants is referred to as \POM.
% 
% We compare the effect on accuracy when adding one of the variants to the backbone (just after the last residual block). \autoref{tab:CA_variations} demonstrates this assessment.
% 
% %------------------------------------------------------------------------------
% \begin{table}
% \centering
% %\resizebox{\columnwidth}{!}{%
% \scriptsize
% \begin{tabular}{lcc}\\\toprule
% 	\Th{Block Type}&\Th{$\#$Params}&\Th{Acc}\\\midrule
% 	CA&4.20M&74.63\\
% 	Proj$\rightarrow$CA&12.58M&74.19\\
% 	CA$\rightarrow$MLP&20.97M&-\\
% 	Proj$\rightarrow$CA$\rightarrow$MLP&29.36M&-\\\bottomrule
% \end{tabular}
% %}
% \vspace{3pt}
% \caption{Comparison of classification performance when one cross attention block is added into the last residual block of ResNet-50.}
% \label{tab:CA_variations}
% \end{table}
% %------------------------------------------------------------------------------
% 
% We observe that the introduction of the basic design of the cross attention module outperforms the classification properties of that which uses projection of the input features to compute the subsequent representation. We hypothesize that maintaining the features without any projection allows the [class] token to better collect global information, as patch information is maintained in the same space that the already trained classifier relies on to perform classification. 
% On another hand, we also note that the introduction of an MLP to update said representation is not feasible given instability during training, for this reason we decide not to pursue further experimentation with this idea.

%------------------------------------------------------------------------------
\begin{table}
\centering
\scriptsize
%\resizebox{\columnwidth}{!}{%}
\begin{tabular}{lcc}\toprule
	\Th{Block Type}&\Th{$\#$Params}&\Th{Accuracy}\\\midrule
	\our&6.96M&74.70\\
	\PO&18.13M&74.41\\\bottomrule
\end{tabular}
%}
%\vspace{3pt}
\caption{\emph{Different cross attention block design for \Ours.} Classification accuracy and parameters using ResNet-50 on ImageNet. \Th{$\#$Param}: parameters of \Ours only.}
\label{tab:dif_streams}
\end{table}
%------------------------------------------------------------------------------

Results are reported in \autoref{tab:dif_streams}. We observe that the stream made of vanilla CA blocks~\eq{CA} offers slightly better accuracy than projections~\eq{proj_ca}, while having less parameters. We also note that most of the computation takes place in the last residual stages, where the channel dimension is the largest. To keep our design simple, we choose the vanilla solution without projections~\eq{CA} by default.

%------------------------------------------------------------------------------

\paragraph{\Ours placement}
\label{ab:placement}

To validate the design of \Ours, we measure the effect of its depth on its performance \vs the baseline \gap in terms of both classification accuracy / number of parameters and classification metrics for interpretability. In particular, we place the stream in parallel to the network $f$, starting at stage $\ell$ and running through stage $L$, the last stage of $f$, where $0 \le \ell \le L$. Results are reported in \autoref{tab:intrecog-resnet}.

%------------------------------------------------------------------------------
\begin{table}
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
%\resizebox{\columnwidth}{!}{%}
\begin{tabular}{lcccccc}\toprule
	\mc{7}{\Th{Accuracy and Parameters}}\\\midrule
	&\Th{Placement}&\mc{2}{\Th{CLS dim}}&\mc{2}{\Th{\#Param}}&\Th{Acc$\uparrow$}\\\midrule
	
	&$S_0-S_4$&\mc{2}{$64$}  &\mc{2}{6.96M}&\textbf{74.70}\\  % 6.963.264
	&$S_1-S_4$&\mc{2}{$256$} &\mc{2}{6.95M}&74.67\\           % 6.947.072
	&$S_2-S_4$&\mc{2}{$512$} &\mc{2}{6.82M}&74.67\\           % 6.816.256
	&$S_3-S_4$&\mc{2}{$1024$}&\mc{2}{6.29M}&74.67\\           % 6.292.480
	&$S_4-S_4$&\mc{2}{$2048$}&\mc{2}{4.20M}&74.63\\\midrule   % 4.196.352
	
	\mc{7}{\Th{Interpretability Metrics}}\\\midrule
	\Th{Method}&\Th{Placement}&\Th{AD$\downarrow$}&\Th{AG$\uparrow$}&\Th{AI$\uparrow$}&\Th{I$\uparrow$}&\Th{D$\downarrow$}\\\midrule
	
	\mr{5}{\Th{Grad-CAM}}&$S_0-S_4$&\textbf{12.54}&\textbf{22.67}&48.56&75.53&13.50\\ % Checked
		&$S_1-S_4$&12.69&22.65&48.31&75.53&13.41\\ % Checked
		&$S_2-S_4$&\textbf{12.54}&21.67&\textbf{48.58}&75.54&13.50\\ % Running
		&$S_3-S_4$&12.69&22.28&47.89&\textbf{75.55}&13.40\\ % Running
		&$S_4-S_4$&12.77&20.65&47.14&74.32&\textbf{13.37}\\\midrule % Checked
		
	\mr{5}{\Th{Grad-CAM++}}&$S_0-S_4$&13.99&19.29&44.60&75.21&13.78\\ % Checked
		&$S_1-S_4$&13.99&19.29&44.62&75.21&13.78\\ % Checked
		&$S_2-S_4$&13.71&\textbf{19.90}&\textbf{45.43}&75.34&13.50\\ % Running
		&$S_3-S_4$&13.69&19.61&45.04&\textbf{75.36}&13.50\\ % Running
		&$S_4-S_4$&\textbf{13.67}&18.36&44.40&74.19&\textbf{13.30}\\\midrule % Checked
		
	\mr{5}{\Th{Score-CAM}}&$S_0-S_4$&\textbf{7.09}&23.65&54.20&74.91&14.68\\ % Checked
		&$S_1-S_4$&\textbf{7.09}&23.65&54.20&74.92&14.68\\ % Checked
		&$S_2-S_4$&\textbf{7.09}&\textbf{23.66}&\textbf{54.21}&74.91&14.68\\ % Running
		&$S_3-S_4$&7.74&23.03&52.92&\textbf{74.97}&14.65\\ % Running
		&$S_4-S_4$&7.52&19.45&50.45&74.19&\textbf{14.46}\\\bottomrule % Checked
\end{tabular}
% }
%\vspace{3pt}
\caption{\emph{Effect of stream placement} on accuracy, parameters and interpretability metrics  for ResNet-50 on ImageNet. $S_\ell-S_L$: \Ours runs from stage $\ell$ to $L$ (last); \Th{$\#$Param}: parameters of \Ours only.}
\label{tab:intrecog-resnet}
\end{table}
%------------------------------------------------------------------------------

From the interpretability metrics as well as accuracy, we observe that stream configurations that allow for iterative interaction with the network features obtain the best performance, although the effect of stream placement is small in general. In many cases, the lightest stream of only one cross attention block ($S_4-S_4$) is inferior to options allowing for more interaction. 
Since starting the stream at early stages has little effect on the number of parameters and performance is stable, we choose to start the stream in the first stage ($S_0-S_4$) by default.

%------------------------------------------------------------------------------



%------------------------------------------------------------------------------

%% Top design, bottom interp metrics
%% More parts for experiments

% Ablation of histogram of diferences with extreme cases


==> WACV_Backups/tex_wacv/exp_interp.tex <==
\subsection{Interpretabity metrics}
\label{subsec:interecon}

%------------------------------------------------------------------------------
\begin{table}
\centering
\scriptsize
\setlength{\tabcolsep}{3.5pt}
% \resizebox{\columnwidth}{!}{%
\begin{tabular}{llcccccc}\toprule
	\mc{8}{\Th{Accuracy and Parameters}}\\\midrule
	\Th{Network}&\mc{1}{\Th{Pool}}&\Th{GFLOPs}&\mc{2}{\Th{$\#$Param}}&\mc{2}{\Th{Param$\%$}}&\Th{Acc$\uparrow$}\\\midrule
	\mr{2}{\Th{ResNet-18}}&\mc{1}{\gap}&3.648&\mc{2}{11.69M}&\mc{2}{\mr{2}{3.71}}&67.28\\
		&\mc{1}{\ours}&3.652&\mc{2}{12.13M}&&&67.54\\\midrule
	\mr{2}{\Th{ResNet-50}}&\mc{1}{\gap}&8.268&\mc{2}{25.56M}&\mc{2}{\mr{2}{27.27}}&74.55\\
		&\mc{1}{\ours}&8.288&\mc{2}{32.53M}&&&74.70\\\midrule
	\mr{2}{\Th{ConvNeXt-S}}&\mc{1}{\gap}&17.395&\mc{2}{50.22M}&\mc{2}{\mr{2}{1.95}}&83.26\\
		&\mc{1}{\ours}&17.400&\mc{2}{51.20M}&&&83.14\\\midrule
	\mr{2}{\Th{ConvNeXt-B}}&\mc{1}{\gap}&30.747&\mc{2}{88.59M}&\mc{2}{\mr{2}{1.96}}&83.72\\
		&\mc{1}{\ours}&30.753&\mc{2}{90.33M}&&&83.51\\\midrule
%	\mr{2}{\Th{ViT-Base}}&&\cls\footnotemark{}&\mc{2}{86.58M}&\mc{2}{\mr{2}{8.18}}&80.01\\
%		&&\ours&\mc{2}{93.66M}&&&74.73\\\midrule
		
	\mc{8}{\Th{Interpretability Metrics}}\\\midrule
	\Th{Network}&\Th{Method}&\Th{Pool}&\Th{AD$\downarrow$}&\Th{AG$\uparrow$}&\Th{AI$\uparrow$}&\Th{I$\uparrow$}&\Th{D$\downarrow$}\\\midrule

	\mr{7}{\Th{ResNet-18}}&\mr{2}{Grad-CAM}&\gap&17.64&12.73&41.21&63.13&\textbf{10.66}\\ %
		& &\ours&\textbf{16.99}&\textbf{17.22}&\textbf{44.95}&\textbf{65.94}&10.68\\\cmidrule{2-8} %
		& \mr{2}{Grad-CAM++}&\gap&19.05&11.16&37.99&62.80&\textbf{10.75}\\ %
		& &\ours&\textbf{19.02}&\textbf{14.76}&\textbf{40.82}&\textbf{65.53}&10.82\\\cmidrule{2-8} %
		& \mr{2}{Score-CAM}&\gap&13.64&12.98&44.53&62.56&\textbf{11.37}\\ %
		& &\ours&\textbf{11.53}&\textbf{18.12}&\textbf{50.32}&\textbf{65.33}&11.51\\\midrule %

	\mr{7}{\Th{ResNet-50}}&\mr{2}{Grad-CAM}&\gap&13.04&17.56&44.47&72.57&\textbf{13.24}\\ %
		& &\ours&\textbf{12.54}&\textbf{22.67}&\textbf{48.56}&\textbf{75.53}&13.50\\\cmidrule{2-8} %
		& \mr{2}{Grad-CAM++}&\gap&\textbf{13.79}&15.87&42.08&72.32&\textbf{13.33}\\ %
		& &\ours&13.99&\textbf{19.29}&\textbf{44.60}&\textbf{75.21}&13.78\\\cmidrule{2-8} %
		& \mr{2}{Score-CAM}&\gap&8.83&17.97&48.46&71.99&\textbf{14.31}\\ %
		& &\ours&\textbf{7.09}&\textbf{23.65}&\textbf{54.20}&\textbf{74.91}&14.68\\\midrule%

	% \multirow{6}{*}{MobileNet-V2}&\mc{2}{Grad-CAM}&\gap&16.11&12.89&40.27&64.47&\textbf{11.92}\\
	%   & &\ours&\textbf{15.53}&\textbf{16.13}&\textbf{42.95}&\textbf{67.80}&12.24\\\cmidrule{2-8}
	%   & \mc{2}{Grad-CAM++}&\gap&17.65&11.12&37.30&64.08&\textbf{11.96}\\
	%   & &\ours&\textbf{17.55}&\textbf{13.52}&\textbf{38.61}&\textbf{67.36}&12.28\\\cmidrule{2-8}
	%   & \mc{2}{Score-CAM}&\gap&12.32&13.52&43.94&64.13&\textbf{12.23}\\
	%   & &\ours&\textbf{10.71}&\textbf{17.35}&\textbf{47.81}&\textbf{67.41}&12.65\\\midrule

	% \multirow{6}{*}{ConvNext Tiny}&\mc{2}{Grad-CAM}&\gap&43.15&2.82&16.58&49.15&\textbf{23.68}\\ % Numbers match, check saliency
	%   & &\ours&\textbf{22.49}&\textbf{14.03}&\textbf{30.65}&\textbf{82.55}&35.22\\\cmidrule{2-8} % Revision running
	%   & \mc{2}{Grad-CAM++}&\gap&43.96&2.45&15.67&48.95&\textbf{23.90}\\ % Pending
	%   & &\ours&\textbf{25.90}&\textbf{12.16}&\textbf{27.70}&\textbf{82.01}&40.42\\\cline{2-8} % Revision running
	%   & \mc{2}{Score-CAM}&\gap&48.25&1.86&13.47&47.12&\textbf{35.38}\\ % Pending
	%   & &\ours&\textbf{19.69}&\textbf{12.42}&\textbf{28.92}&\textbf{80.21}&49.25\\\midrule % Revision running

	\mr{7}{\Th{ConvNeXt-S}}&\mr{2}{Grad-CAM}&\gap&42.99&1.69&12.60&48.42&\textbf{30.12}\\ % Numbers match, check saliency
		& &\ours&\textbf{22.09}&\textbf{14.91}&\textbf{32.65}&\textbf{84.82}&43.02\\\cmidrule{2-8} % Revision running
		& \mr{2}{Grad-CAM++}&\gap&56.42&1.32&10.35&48.28&\textbf{33.41}\\ % Pending
		& &\ours&\textbf{51.87}&\textbf{9.40}&\textbf{20.55}&\textbf{84.28}&52.58\\\cmidrule{2-8} % Revision running
		& \mr{2}{Score-CAM}&\gap&74.79&1.29&10.10&47.40&\textbf{38.21}\\ % Pending
		& &\ours&\textbf{64.21}&\textbf{8.81}&\textbf{18.96}&\textbf{82.92}&57.46\\\midrule % Revision running

	\mr{7}{\Th{ConvNeXt-B}}&\mr{2}{Grad-CAM}&\gap&33.72&2.43&15.25&52.85&\textbf{29.57}\\ % Pending
		& &\ours&\textbf{19.45}&\textbf{13.96}&\textbf{32.89}&\textbf{86.38}&45.29\\\cmidrule{2-8} % Revision running
		& \mr{2}{Grad-CAM++}&\gap&\textbf{34.01}&2.37&15.60&52.83&\textbf{29.17}\\ % Pending
		& &\ours&36.69&\textbf{8.00}&\textbf{21.95}&\textbf{85.39}&53.42\\\cmidrule{2-8} % Revision running
		& \mr{2}{Score-CAM}&\gap&43.55&2.23&15.67&50.96&\textbf{39.49}\\ % Pending
		& &\ours&\textbf{23.51}&\textbf{11.04}&\textbf{27.35}&\textbf{83.41}&60.53\\\midrule% Revision running

%	\mr{7}{\Th{ViT-B}}&\mr{2}{Grad-CAM}&\cls\footnotemark[\value{footnote}]&83.66&1.49&7.37&66.43&34.98\\ % Pending
%		& &\ours&49.88&4.07&16.10&67.12&10.25\\\cmidrule{2-8} % Revision running
%		& \mr{2}{Grad-CAM++}&\cls\footnotemark[\value{footnote}]&97.03&0.01&1.36&\textbf{66.80}&33.35\\ % Pending
%		& &\ours&74.81&1.64&7.43&61.95&28.29\\\cmidrule{2-8} % Revision running
%		& \mr{2}{Score-CAM}&\cls\footnotemark[\value{footnote}]&TBA&TBA&TBA&TBA&TBA\\ % Pending
%		& &\ours&TBA&TBA&TBA&TBA&TBA\\\bottomrule % Revision running
\end{tabular}
% }
%\vspace{3pt}
\caption{\emph{Accuracy, parameters and interpretability metrics} of \Ours \vs baseline \gap for different networks and interpretability methods on ImageNet. \Th{$\#$Param}: total parameters; \Th{Param$\%$}: percentage of \Ours parameters relative to backbone.}
\label{tab:intrecon-all}
\end{table}
%------------------------------------------------------------------------------
% \footnotetext{Built-in \cls token from Vision Transformers.}    
%------------------------------------------------------------------------------

Here we measure the effect of employing our \Ours approach to pool features \vs the baseline \gap on the faithfulness of explanations, using classification metrics for interpretability. Results are reported in \autoref{tab:intrecon-all} for ImageNet and  \autoref{tab:pascal} for CUB and Pascal VOC.

\autoref{tab:intrecon-all} shows that for different networks, CAM-based interpretability methods and dataset, \Ours provides consistent improvements over \gap in terms of AD, AG, AI and I metrics, while performing lower on D. 
%
%\textcolor{red}{
Deletion has raised concerns in previous works \cite{chefer2021transformer, zhang2023opti}. Indeed, it gradually replaces pixels by black, unlike insertion which starts from a blurred image. This poses the problem of \emph{out-of-distribution} (OOD) data~\cite{gomez2022metrics, hase2021outofdistribution, qiu2021resisting}, possibly introducing bias related to the shape of black regions~\cite{rong2022consistent}. Moreover, non-spread saliency maps tend to perform better \cite{zhang2023opti}, which is likely the reason for lower performance. %We suppose that erasing one main object area is more efficient.  
%}

%\textcolor{orange}{Considering that saliency maps of the two pooling methods do not present large differences, the observed improvement in interpretability metrics can be attributed to the predictive power of the learned attention mechanism. 
%}

%That is, class probabilities can change due to attention, even if saliency maps, obtained features and predictions are the same.}
%\textcolor{red}{
Results on CUB in \autoref{tab:pascal} show that our \Ours consistently provides improvements when the model is finetuned on a smaller fine-grained dataset.
%}

%Table \autoref{tab:pascal} present interpretability results for the PASCAL dataset \cite{Everingham15}.
% \textcolor{red}{
Regarding Pascal VOC, the results for Score-CAM are similar to the ones on ImageNet and CUB, with consistent improvements on all metrics but Deletion. 
However, Grad-CAM and Grad-CAM++ only provide improvements on Average Gain and Average Increase. Average Drop, Insertion and Deletion are very similar.
In fact, Pascal VOC is a multi-class dataset and  our \Ours is class agnostic. Thus, the attention-based pooling is the same for different class for a given image, which reduces the benefit of our \Ours.
%We believe the fact that 
% }

It is also interesting to observe the performance of Score-CAM, as it computes channel weights $\alpha_k^c$ in~\eq{sal} without using gradients. 
In gradient-based methods, channel weights are modified by \Ours due to modified backward gradient flow to features through cross attention blocks rather than \gap.
In Score-CAM however, channel weights are only modified in the forward class probabilities computation, due to attention.

% Regarding the results on ViT-Base, we observe the previously reported failure of CAM based methods on vision transformers\cite{zhang2023opti,chefer2021transformer}; in contrast we note that with the addition of our stream, the interpretability properties \textbf{changes.}

%------------------------------------------------------------------------------

% \subsection{Localization Evaluation}
% \label{subsec:loceval}
% 
% In this section, we assess the localization properties of the saliency maps provided by the inclusion of the CLS stream-based representation. We report these results in table \ref{tab:localization}. It shows that all the localization metrics provide similar scores on different methods and networks. CLS helps saliency maps keep localization information while gaining more classification information. 
% \begin{table}[H]
% 	\centering
% 	%\resizebox{\columnwidth}{!}{%
% 	\scriptsize
% 	\setlength{\tabcolsep}{2pt}
% 	\begin{tabular}{lllccc|cccc}\toprule
% 		\Th{Backbone}&\Th{Method}&\Th{Repr}&\Th{OM$\downarrow$}&\Th{LE$\downarrow$}&\Th{F1$\uparrow$}&\Th{BA$\uparrow$}&\Th{SP$\uparrow$}&\Th{EP$\uparrow$}&\Th{SM$\downarrow$}\\\midrule
% 		\mr{6}{\Th{ResNet-18}}&\mr{2}{\Th{Grad-CAM}}&GAP&\tb{80.6}&61.4&49.1&\tb{58.3}&13.7&13.1&\tb{2.93}\\
% 			& &CLS&81.1&\tb{61.3}&49.1&58.2&13.7&13.1&3.10\\ \cmidrule{3-10}
% 			&\mr{2}{\Th{Grad-CAM++}}&GAP&\tb{80.5}&60.9&50.0&\tb{58.3}&13.7&13.1&\tb{2.89}\\
% 			& &CLS&81.0&60.9&\tb{50.1}&58.0&13.7&13.1&3.07\\\cmidrule{3-10}
% 			&\mr{2}{\Th{Score-CAM}}&GAP&\tb{80.5}&60.9&\tb{49.7}&57.7&13.7&13.1&\tb{2.89}\\
% 			& &CLS&81.0&60.9&49.5&57.3&13.7&13.1&3.07\\ \midrule
% 			\mr{6}{\Th{ResNet-50}}&\mr{2}{\Th{Grad-CAM}}&GAP&80.0&66.4&49.5&58.8&13.8&13.2&\tb{2.56}\\
% 			& &CLS&80.0&66.4&\tb{49.6}&58.8&13.8&13.2&2.62\\\cmidrule{3-10}
% 			&\mr{2}{\Th{Grad-CAM++}}&GAP&\tb{80.2}&\tb{66.7}&50.4&\tb{58.7}&13.9&13.3&\tb{2.55}\\
% 			& &CLS&80.3&66.9&\tb{50.6}&58.0&13.9&13.3&2.64\\\cmidrule{3-10}
% 			&\mr{2}{\Th{Score-CAM}}&GAP&\tb{80.0}&66.3&\tb{50.3}&\tb{57.9}&13.8&13.2&\tb{2.55}\\
% 			& &CLS&80.1&66.3&50.0&57.5&13.8&13.2&2.62\\\bottomrule
% 	\end{tabular}
% 	%}
% 	\caption{Comparison of interpretable localization for ResNet on ImageNet.}
% 	\label{tab:localization}
% \end{table}

%------------------------------------------------------------------------------

\subsection{Classification accuracy}
\label{subsec:classification}

%Here we measure the effect of employing our \Ours approach to pool features \vs the baseline \gap on 

Classification accuracy, number of parameters and GFLOPs for both our \Ours and the baselines are reported in \autoref{tab:intrecon-all} (top part).

By adding our \Ours to the network, classification remains on par with the baseline. Importantly, the network including the classifier remains frozen and the features used for the global image representation remain fixed, meaning that any change in accuracy is due to the attention-based pooling mechanism. 
%
% \textcolor{red}{
We further report the number of GFLOPs for one forward pass and the parameters count of both methods.
Our \Ours has little computation cost and the parameter overhead depends on the embedding dimension because of projection $W_\ell$ in~\eq{qk-layer} and is small in general, except for ResNet-50. Thus, with small overhead in resources, \Ours achieves superior explanations of the classifier predictions, while maintaining accuracy.
% }

%------------------------------------------------------------------------------
\begin{table}
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
%\resizebox{\columnwidth}{!}{%
\begin{tabular}{llccccc}\toprule                    
	\mc{7}{\textbf{\Th{CUB-200-2011 - ResNet-50}}}\\\midrule
	&\Th{Pooling}&\mc{2}{}&\mc{2}{}&\Th{Acc$\uparrow$}\\\midrule
		&\gap&\mc{2}{}&\mc{2}{}&76.96\\
		&\ours&\mc{2}{}&\mc{2}{}&75.90\\\midrule
	
	\mc{7}{\Th{Interpretability Metrics}}\\\midrule
	\Th{Method}&\Th{Pooling}&AD$\downarrow$&AG$\uparrow$&AI$\uparrow$&I$\uparrow$&D$\downarrow$\\\midrule
	% \multirow{3}{*}{GAP}&\multirow{3}{*}{74.55}&Grad-CAM&13.04&17.56&44.47&72.57&13.24\\
	%  & &Grad-CAM++&13.79&15.87&42.08&72.32&13.33\\
	%  & &Score-CAM&13.64&12.98&44.53&62.56&11.37\\\hline %
	\mr{2}{Grad-CAM}&\gap&10.87&10.29&45.81&65.71&\textbf{6.17}\\
		&\ours&\textbf{10.44}&\textbf{17.61}&\textbf{53.54}&\textbf{74.60}&6.56\\\midrule
	\mr{2}{Grad-CAM++}&\gap&11.35&9.68&44.32&65.64&\textbf{5.92}\\
		&\ours&\textbf{11.01}&\textbf{16.50}&\textbf{51.63}&\textbf{74.64}&6.21\\\midrule
	\mr{2}{Score-CAM}&\gap&9.05&10.62&48.90&65.58&5.94\\
		&\ours&\textbf{6.37}&\textbf{19.50}&\textbf{60.41}&\textbf{74.22}&\textbf{2.14}\\

\midrule
  \midrule

	\mc{7}{\textbf{\Th{Pascal VOC 2012 - ResNet-50}}}\\\midrule
	&\Th{Pooling}&\mc{2}{}&\mc{2}{}&\Th{mAP$\uparrow$}\\\midrule
		&\gap&\mc{2}{}&\mc{2}{}&78.32\\
		&\ours&\mc{2}{}&\mc{2}{}&78.35\\\midrule
	
	\mc{7}{\Th{Interpretability Metrics}}\\\midrule
	\Th{Method}&\Th{Pooling}&AD$\downarrow$&AG$\uparrow$&AI$\uparrow$&I$\uparrow$&D$\downarrow$\\\midrule
	% \multirow{3}{*}{GAP}&\multirow{3}{*}{74.55}&Grad-CAM&13.04&17.56&44.47&72.57&13.24\\
	%  & &Grad-CAM++&13.79&15.87&42.08&72.32&13.33\\
	%  & &Score-CAM&13.64&12.98&44.53&62.56&11.37\\\hline %
	\mr{2}{Grad-CAM}&\gap&\textbf{12.61}&9.68&27.88&\textbf{89.10}&59.39\\
		&\ours&12.77&\textbf{15.46}&\textbf{34.53}&88.53&\textbf{59.16}\\\midrule
	\mr{2}{Grad-CAM++}&\gap&\textbf{12.25}&9.68&27.62&\textbf{89.34}&54.23\\
		&\ours&12.28&\textbf{16.76}&\textbf{34.87}&89.02&\textbf{53.34}\\\midrule
	\mr{2}{Score-CAM}&\gap&14.8&6.76&36.41&71.10&\textbf{39.95}\\
		&\ours&\textbf{10.96}&\textbf{21.35}&\textbf{43.82}&\textbf{89.21}&51.44\\\bottomrule
  
\end{tabular}
%}
%\vspace{3pt}
\caption{Accuracy, respectively mean Average Precision, and interpretability metrics of \Ours \vs baseline \gap for ResNet-50 on CUB and Pascal dataset.}
\label{tab:pascal}
\end{table}
%------------------------------------------------------------------------------


==> WACV_Backups/tex_wacv/exp_qual-1.tex <==
%------------------------------------------------------------------------------
\begin{figure*}[t]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{ccccccccc}
        {}&\multirow{2}{*}{Original}&\multirow{2}{*}{Raw Attention}&\multicolumn{2}{c}{Grad-CAM}&\multicolumn{2}{c}{Grad-CAM++}&\multicolumn{1}{c}{Score-CAM}\\
        {}&{}&{}&GAP&CLS&GAP&CLS&GAP&CLS\\
        {\rotatebox{90}{\small Waffle Iron}}&\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1_revisit/original/15749.jpeg}&\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1_revisit/raw_att/15749.jpeg}&\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1_revisit/shelf_gradcam/15749.jpeg}&\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1_revisit/gradcam/15749.jpeg}&\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1_revisit/shelf_gradcampp/15749.jpeg}&\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1_revisit/gradcampp/15749.jpeg}&\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1_revisit/scorecam/15749.jpeg}&\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1_revisit/scorecam/15749.jpeg}\\

        {\rotatebox{90}{\small Wallaby}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1_revisit/original/24263.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1_revisit/raw_att/24263.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1_revisit/shelf_gradcam/24263.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1_revisit/gradcam/24263.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1_revisit/shelf_gradcampp/24263.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1_revisit/gradcampp/24263.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1_revisit/scorecam/24263.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1_revisit/scorecam/24263.jpeg}}\\

        {\rotatebox{90}{\small Hoopskirt}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1_revisit/original/33003.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1_revisit/raw_att/33003.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1_revisit/shelf_gradcam/33003.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1_revisit/gradcam/33003.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1_revisit/shelf_gradcampp/33003.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1_revisit/gradcampp/33003.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1_revisit/scorecam/33003.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1_revisit/scorecam/33003.jpeg}}\\

        {\rotatebox{90}{\small Matchstick}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1_revisit/original/48096.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1_revisit/raw_att/48096.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1_revisit/shelf_gradcam/48096.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1_revisit/gradcam/48096.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1_revisit/shelf_gradcampp/48096.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1_revisit/gradcampp/48096.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1_revisit/scorecam/48096.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1_revisit/scorecam/48096.jpeg}}\\

        {\rotatebox{90}{Sweatshirt}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/original/18939.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/raw_att/18939.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/shelf_gradcam/18939.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/gradcam/18939.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/shelf_gradcampp/18939.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/gradcampp/18939.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/shelf_scorecam/18939.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/scorecam/18939.jpeg}}\\

        {\rotatebox{90}{\small CRT screen}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/original/43057.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/raw_att/43057.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/shelf_gradcam/43057.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/gradcam/43057.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/shelf_gradcampp/43057.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/gradcampp/43057.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/shelf_scorecam/43057.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/scorecam/43057.jpeg}}\\ % Checked 
    \end{tabular}
     }
    \caption{Comparison of saliency maps generated by different CAM methods, using GAP or CLS pooling}
    \label{fig:compmethods}
\end{figure*}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------

\subsection{Qualitative evaluation}
\label{subsec:vinspection}

%% UNDER REVISION
\ronan{We evaluate the quality of saliency maps obtained by  Grad-CAM, Grad-CAM++, and Score-CAM using either [cls] or \gap before the classifier. Moreover, we display the class-agnostic raw attention obtained with [cls], see \autoref{fig:compmethods}.

We observe that raw attention focus on objects of interest in the images.
Moreover the CAM-based techniques have similar saliency maps when using \gap and [cls], as they share the same features maps $F^k_\ell$ and only the weight coefficients $\alpha^c_k$ are modified.
In general, we observe that saliency maps with [cls] tends to cover larger regions of the object or more instances.
The following qualitative experiments show that these changes in saliency maps have a significant impact on the interpretability performances.}

\ronanc{DO WE ADD ATTENTION ONLY ON DATA FROM OTHER DATASETS}

% \input{tex/figure_ra-passes}

%We observe a high degree of similarity between the class-specific explanation maps generated by using both representations. 
%This phenomenon is explained to a great degree by the computation of the weighting coefficient used for CAM methods, as the main factor contributing to these similarities lies within the predictive power of the network, which by itself is affected by the representation used to classify. 
%\autoref{subsec:classification} provides \ronanc{check or clarify the following paragraph maybe} a more concrete explanation of this phenomena. We also observe a contrast between these explanation maps and that produced by attention itself; we note that this representation while covering bigger regions of the image on most instances, presents the most salient points over the object of interest. Ultimately this attention map is used to compute the global representation to classify with.







%///////////////////////////////////old stuff
% We observe that the class-agnostic representation demonstrated by raw-attention, in general covers most of the object of interest of the image,
% We evaluate the quality of the visualizations obtained when using [cls] in comparison to \gap as a representation for classification in \autoref{fig:compmethods}. For this, we compare the class agnostic saliency map obtained by raw attention, and the contrast between Grad-CAM, Grad-CAM++ and ScoreCAM when their computation is carried on using either \gap or [cls].
% In this section, we evaluate the saliency maps generated when we apply the previously mentioned interpretability methods to our approach, in comparison to the baseline models.
% As can be observed on \autoref{fig:compmethods}, the explanation maps generated with the CLS pooling mechanism present a high degree of similarity with those computed using GAP.\\%Conversely on Figure \textit{figure different classes} we observe that our pooling protocol is able to \red{contribution for different classes} when we visualize saliency maps of different categories. Finally, on Figure \textit{contribution towards localization}, we observe that \green{changes on localization given by the application of CLS}.\\
% % We observe that there exists a key factor towards obtaining different saliency maps while following the same interpretability approach.
% % Following our approach and the preservation of the backbone properties, we hypothesize that the small differences obtained for the aforementioned maps are derived from the computation of the weighting coefficient $w_k^c$ previously mentioned in equation \ref{eq:gcam}. Moreover, this coefficient is directly affected by changes on the predictive power for a given network; which on itself can be altered in the same time by the representation of the input image used to classify, be it the GAP features or the [CLS] token. A more detailed explanation of this phenomenon is found in Sections \ref{subsec:interecon} and \ref{subsect:classification}.
% Following our approach and the preservation of the backbone properties, we hypothesize that the small differences observed are derived from the computation of the weighting coefficient $w_k^c$ previously mentioned in equation ~\eq{sal}. Moreover, this coefficient is directly affected by changes on the predictive power for a given network; which on itself is altered at the same time by the representation of the input image used to classify, be it the GAP features or the [CLS] token. A more detailed explanation of this phenomenon is found in \autoref{subsec:interecon} and \autoref{subsect:classification}.
%Sections \ref{subsec:interecon} and \ref{subsect:classification}.

%We hypothesize that while we retain the backbone and classifier layers from the baseline model, the different representations are derived from the computation of the weighting coefficient $w_k^c$ previously mentioned in Equation \ref{eq:gcam}. We note that while we compare explanations provided by the same network and saliency method, the computation of this coefficient is directly affected due changes on the predictive power of the model, which is given by the kind of representation that is used to classify. A more detailed explanation of this phenomenon is found in Sections \ref{subsec:interecon} and \ref{subsect:classification}.

% \begin{figure*}[t]
%     \centering
%     \resizebox{\textwidth}{!}{%
%     \begin{tabular}{ccccccccc}
%         {}&\multirow{2}{*}{Original}&\multirow{2}{*}{Raw Attention}&\multicolumn{2}{c}{Grad-CAM}&\multicolumn{2}{c}{Grad-CAM++}&\multicolumn{1}{c}{Score-CAM}\\
%         {}&{}&{}&GAP&CLS&GAP&CLS&GAP&CLS\\
%         {\rotatebox{90}{\small Car Mirror}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/original/351.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/raw_att/351.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/shelf_gradcam/351.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/gradcam/351.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/shelf_gradcampp/351.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/gradcampp/351.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/shelf_scorecam/351.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/scorecam/351.jpeg}}\\ % Checked for ordering

%         {\rotatebox{90}{\small Sea Cucumber}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/original/18852.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/raw_att/18852.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/shelf_gradcam/18852.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/gradcam/18852.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/shelf_gradcampp/18852.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/gradcampp/18852.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/shelf_scorecam/18852.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/scorecam/18852.jpeg}}\\ %% Checked for ordering

%         {\rotatebox{90}{Sweatshirt}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/original/18939.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/raw_att/18939.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/shelf_gradcam/18939.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/gradcam/18939.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/shelf_gradcampp/18939.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/gradcampp/18939.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/shelf_scorecam/18939.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/scorecam/18939.jpeg}}\\

%         {\rotatebox{90}{Bobsled}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/original/20604.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/raw_att/20604.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/gradcam/20604.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/shelf_gradcam/20604.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/gradcampp/20604.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/shelf_gradcampp/20604.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/scorecam/20604.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/shelf_scorecam/20604.jpeg}}\\%Small differences
             
%         {\rotatebox{90}{Beaver}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/original/28492.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/raw_att/28492.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/gradcam/28492.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/shelf_gradcam/28492.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/gradcampp/28492.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/shelf_gradcampp/28492.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/scorecam/28492.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/shelf_scorecam/28492.jpeg}}\\ % Small differences
              
%         {\rotatebox{90}{\small CRT screen}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/original/43057.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/raw_att/43057.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/shelf_gradcam/43057.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/gradcam/43057.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/shelf_gradcampp/43057.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/gradcampp/43057.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/shelf_scorecam/43057.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.175\textwidth]{Images/Comparable/figure1/scorecam/43057.jpeg}}\\ % Checked 
%     \end{tabular}
%     }
%     \caption{Comparison of saliency maps generated by different CAM methods, using GAP or CLS pooling}
%     \label{fig:compmethods}
% \end{figure*}
% \subsection{Qualitative Evaluation}
% \label{subsec:vinspection}

==> WACV_Backups/tex_wacv/exp_qual.tex <==
%------------------------------------------------------------------------------
\begin{figure*}[t]
\scriptsize
\centering
\setlength{\tabcolsep}{1.5pt}
% \resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccccc}
	{}&\multirow{2}{*}{Input image}&\multirow{2}{*}{Raw Attention}&\multicolumn{2}{c}{Grad-CAM}&\multicolumn{2}{c}{Grad-CAM++}&\multicolumn{1}{c}{Score-CAM}\\
	{}&{}&{}&GAP&\Ours&GAP&\Ours&GAP&\Ours\\
    % {\rotatebox{90}{\tiny Loudspeaker}}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_similarities/original/37729.jpeg}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_similarities/raw_att/37729.jpeg}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_similarities/shelf_gradcam/37729.jpeg}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_similarities/gradcam/37729.jpeg}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_similarities/shelf_gradcampp/37729.jpeg}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_similarities/gradcampp/37729.jpeg}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_similarities/scorecam/37729.jpeg}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_similarities/shelf_scorecam/37729.jpeg}\\

    {\rotatebox{90}{\tiny Envelope}}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_similarities/original/23541.jpeg}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_similarities/raw_att/23541.jpeg}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_similarities/shelf_gradcam/23541.jpeg}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_similarities/gradcam/23541.jpeg}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_similarities/shelf_gradcampp/23541.jpeg}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_similarities/gradcampp/23541.jpeg}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_similarities/scorecam/23541.jpeg}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_similarities/shelf_scorecam/23541.jpeg}\\

    {\rotatebox{90}{\tiny Groom}}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_similarities/original/9602.jpeg}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_similarities/raw_att/9602.jpeg}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_similarities/shelf_gradcam/9602.jpeg}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_similarities/gradcam/9602.jpeg}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_similarities/shelf_gradcampp/9602.jpeg}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_similarities/gradcampp/9602.jpeg}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_similarities/scorecam/9602.jpeg}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_similarities/shelf_scorecam/9602.jpeg}\\

    {\rotatebox{90}{\tiny Nematode}}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_similarities/original/12414.jpeg}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_similarities/raw_att/12414.jpeg}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_similarities/shelf_gradcam/12414.jpeg}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_similarities/gradcam/12414.jpeg}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_similarities/shelf_gradcampp/12414.jpeg}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_similarities/gradcampp/12414.jpeg}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_similarities/scorecam/12414.jpeg}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_similarities/shelf_scorecam/12414.jpeg}\\

	% {\rotatebox{90}{\tiny Waffle Iron}}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_revisit/original/15749.jpeg}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_revisit/raw_att/15749.jpeg}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_revisit/shelf_gradcam/15749.jpeg}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_revisit/gradcam/15749.jpeg}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_revisit/shelf_gradcampp/15749.jpeg}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_revisit/gradcampp/15749.jpeg}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_revisit/scorecam/15749.jpeg}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_revisit/scorecam/15749.jpeg}\\

	% {\rotatebox{90}{\tiny Wallaby}}&\multicolumn{1}{c}{\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_revisit/original/24263.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_revisit/raw_att/24263.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_revisit/shelf_gradcam/24263.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_revisit/gradcam/24263.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_revisit/shelf_gradcampp/24263.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_revisit/gradcampp/24263.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_revisit/scorecam/24263.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_revisit/scorecam/24263.jpeg}}\\

	% {\rotatebox{90}{\tiny Hoopskirt}}&\multicolumn{1}{c}{\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_revisit/original/33003.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_revisit/raw_att/33003.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_revisit/shelf_gradcam/33003.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_revisit/gradcam/33003.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_revisit/shelf_gradcampp/33003.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_revisit/gradcampp/33003.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_revisit/scorecam/33003.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_revisit/scorecam/33003.jpeg}}\\

	% {\rotatebox{90}{\tiny Matchstick}}&\multicolumn{1}{c}{\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_revisit/original/48096.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_revisit/raw_att/48096.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_revisit/shelf_gradcam/48096.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_revisit/gradcam/48096.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_revisit/shelf_gradcampp/48096.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_revisit/gradcampp/48096.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_revisit/scorecam/48096.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_revisit/scorecam/48096.jpeg}}\\

	% {\rotatebox{90}{\tiny Sweatshirt}}&\multicolumn{1}{c}{\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1/original/18939.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1/raw_att/18939.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1/shelf_gradcam/18939.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1/gradcam/18939.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1/shelf_gradcampp/18939.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1/gradcampp/18939.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1/shelf_scorecam/18939.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1/scorecam/18939.jpeg}}\\

	{\rotatebox{90}{\tiny CRT screen}}&\multicolumn{1}{c}{\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1/original/43057.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1/raw_att/43057.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1/shelf_gradcam/43057.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1/gradcam/43057.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1/shelf_gradcampp/43057.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1/gradcampp/43057.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1/shelf_scorecam/43057.jpeg}}&\multicolumn{1}{c}{\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1/scorecam/43057.jpeg}}\\ % Checked 

   {\rotatebox{90}{\tiny Snowboard}}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_similarities/original/11376.jpeg}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_similarities/raw_att/11376.jpeg}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_similarities/shelf_gradcam/11376.jpeg}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_similarities/gradcam/11376.jpeg}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_similarities/shelf_gradcampp/11376.jpeg}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_similarities/gradcampp/11376.jpeg}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_similarities/scorecam/11376.jpeg}&\includegraphics[width=0.115\textwidth]{Images/Comparable/figure1_similarities/shelf_scorecam/11376.jpeg}\\

 
\end{tabular}
% }
\vspace{3pt}
\caption{Comparison of saliency maps generated by different CAM-based methods, using GAP and our \Ours, on ImageNet images. The raw attention is the one used for pooling by \Ours.}
\label{fig:compmethods}
\end{figure*}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------

\subsection{Qualitative evaluation}
\label{subsec:vinspection}

We show saliency maps obtained by different interpretability methods using either \gap or \Ours, as well as the class-agnostic raw attention coming from our \Ours, see \autoref{fig:compmethods}.
%, including the class-agnostic raw attention obtained by \Ours.

We observe that the raw attention focuses on objects of interest in the images. 
%\textcolor{orange}{
In general, saliency maps obtained with \Ours are similar but tend to cover larger regions of the object or more instances compared with \gap.%, see \autoref{fig:compmethods}.
%, for example in the ``CRT screen'' image in \autoref{fig:compmethods}. 
%}
%
Indeed, the differences in saliency maps should not be large, as both methods share the same features maps $F^k_\ell$ and only the weight coefficients $\alpha^c_k$ differ.
Despite the small differences, the following quantitative results show that \Ours has a significant impact on the interpretability metrics.

%
%\textcolor{red}{
%As a further investigation, we compute cosine similarities of saliency maps and obtain 0.998 (or 6.49\% euclidean distance), averaged over the dataset. We then observed a similarity of 0.752 for the pooled features and 0.612 for the gradient.
%Finally, the percentage difference in probability for the ground truth class is of 27.8\% on average.
%These results show that the small changes in the saliency maps are meaningful.
%}


%In some examples, the saliency maps obtained are quite similar.%using \gap and \Ours are not very different. 
%The differences are expected to be low, as both methods share the same features maps $F^k_\ell$ and only the weight coefficients $\alpha^c_k$ differ.
%%, while the CAM-based methods have their own mechanism to focus on what is relevant for the prediction of the class of interest. 
%Despite the small visual differences, the following quantitative results show that \Ours has a significant impact on the interpretability metrics.

%------------------------------------------------------------------------------
\input{tex/figure_outdataset}
%------------------------------------------------------------------------------

In addition, \autoref{fig:enter-label} shows examples of images from the MIT 67 Scenes dataset~\cite{quattoni2009recognizing} along with raw attention maps obtained by \Ours. These images come from four classes that do not exist in ImageNet and the network sees them at inference for the first time. Nevertheless, the attention maps focus on objects of interest in general.


==> WACV_Backups/tex_wacv/exp_setup-1.tex <==
\section{Experiments}
%We evaluate our approach to study the interpretability properties it presents and the effect on classification performance.
In this section, we evaluate the interpretability and recognition properties of our approach. For this goal,  we generate explanations following current state-of-the art post-hoc interpretability methods derived from CAM\cite{DBLP:journals/corr/HeZRS15}; namely Grad-CAM\cite{DBLP:journals/corr/SelvarajuDVCPB16}, Grad-CAM++\cite{DBLP:journals/corr/abs-1710-11063} and most recently ScoreCAM\cite{DBLP:journals/corr/abs-1910-01279}. First, on Section \ref{subsec:setup} we briefly describe the general training regime used to train our approach alongside its variations. Next, we conduct qualitative evaluation for our explanations found in Section \ref{subsec:vinspection}. Afterwards, we assess the fairness of these explanations on image recognition in Section \ref{subsec:interecon}. Moreover, on Section \ref{subsec:loceval} we study their object localization capabilities. On Section \ref{subsect:classification} we compare the classification performance derived from the addition of this attention mechanism to existing models. Lastly, on Section \ref{sec:gen_ablation} we present experiments regarding the design of the CLS Stream and some of its properties.

\subsection{Experimental Setup}\label{subsec:setup}
%We train and evaluate our models on the ImageNet ILSVRC2012 dataset\cite{deng2009imagenet} on the training and validation splits respectively. Since we aim at learning our [CLS] token alongside its interactions with feature maps at different stages of a network; we experiment with pretrained models\footnote{https://pytorch.org/vision/0.8/models.html}, that are used to optimize the CLS stream. During this training phase we learn the parameters of this stream, maintaining the backbone properties intact and leveraging the classifier's predictive power with our representations. Details of this training phase are given in the supplementary material.\\
We train and evaluate our models on the ImageNet ILSVRC-2012 dataset\cite{deng2009imagenet} on the training and validation splits respectively. Since we aim at learning our [CLS] token alongside its interactions with feature maps at different stages of a network; we experiment with pretrained models\footnote{https://pytorch.org/vision/0.8/models.html}, that are used to optimize the CLS stream. During this training phase we learn the parameters of this branch, leveraging its interactions with the backbone and the classifier's predictive power with our representations. Further details of this training phase are given in the supplementary material. \textbf{Maybe here the main recipe for ResNet knowing that its used throughout the ablation}\\

To evaluate our approach and in contrast to similar alternatives assessing interpretability; we use the entirety of the validation set, gaining complete insight on the real performance of our proposed method and its comparisons. To do so, we generate saliency maps of the ensemble of model and CLS stream, that are contrasted with those generated by the application the aforementioned interpretability methods on the model alone.\\  %More details of the experimental set-up


==> WACV_Backups/tex_wacv/exp_setup.tex <==
\section{Experiments}
\label{sec:exp}

We evaluate the interpretability and recognition capabilities of our approach. In particular, we generate explanations following current state-of-the art post-hoc interpretability methods derived from CAM~\cite{zhou2016learning}. We compare the properties of the backbone network $f$ with and without our \Ours, where $f$ is pretrained and fixed.

\subsection{Experimental setup}
\label{subsec:setup}

\paragraph{Training}

We train and evaluate our models on the ImageNet ILSVRC-2012 dataset~\cite{deng2009imagenet}, on the training and validation splits respectively. Thus, we experiment with ResNet-based architectures~\cite{he2016deep} such as ResNet-18 and ResNet-50, and ConvNeXt based architectures~\cite{liu2022convnet} such as ConvNeXt-Small and ConvNeXt-Base. We aim at learning our \Ours, generating a \cls token that interacts with feature maps at different stages of network $f$, to serve as an attention-based pooling mechanism in order to interpret the predictions of $f$. Therefore, we experiment with pretrained models\footnote{https://pytorch.org/vision/0.8/models.html}, that we keep frozen while the parameters of the \Ours are optimized. Details on training hyperparameters are given in the appendix.

Moreover, we present experiments on the bird dataset: CUB-200-2011 \cite{WahCUB_200_2011} and on PASCAL VOC 2012 dataset \cite{Everingham15}. Here the ResNet-50 network is fine-tuned to these dataset as baseline. Then, our \Ours is learned as for ImageNet.

\paragraph{Evaluation}

We employ existing post-hoc interpretability methods to generate saliency maps with and without \Ours and compare interpretability metrics as well as classification accuracy. Regarding interpretability methods, we use Grad-CAM~\cite{DBLP:journals/corr/SelvarajuDVCPB16}, Grad-CAM++~\cite{DBLP:journals/corr/abs-1710-11063} and ScoreCAM~\cite{DBLP:journals/corr/abs-1910-01279}. We note that the evaluation is performed on the entire validation set, unlike the previous approaches.

Following Opti-CAM~\cite{zhang2023opti}, we use a number of classification metrics for interpretability. In particular, we consider the changes in predictive power measured by \emph{average drop} (AD)~\cite{DBLP:journals/corr/abs-1710-11063} and \emph{average gain} (AG)~\cite{zhang2023opti}, the proportion of better explanations measured by \emph{average increase} (AI)~\cite{DBLP:journals/corr/abs-1710-11063} and the impact of different extent of masking measured by \emph{insertion} (I) and \emph{deletion} (D)~\citep{petsiuk2018rise}.

% For localization, we use metrics from the \emph{weakly-supervised object localization} (WSOL) task to measure the maximum overlap between the saliency map (or corresponding predicted bounding boxes) and ground truth bounding boxes, \ie \emph{official metric} (OM), \emph{localization error} (LE), \emph{pixel-wise $F_1$ score}, \emph{box accuracy} (BoxAcc)~\citep{choe2020evaluating} and \emph{saliency metric} (SM)~\citep{dabkowski2017real}. We also measure the localization of the pixel of maximum saliency by the \emph{standard pointing game} (SP)~\cite{zhang2018top} and the fraction of the saliency map within the ground truth bounding boxes by \emph{energy pointing game} (EP)~\citep{DBLP:journals/corr/abs-1910-01279}. We obtain the ground truth bounding boxes from the ILSVRC2014\footnote{\url{https://www.image-net.org/challenges/LSVRC/2014/index\#}} dataset. 




==> WACV_Backups/tex_wacv/exp_var.tex <==
\subsection{Variations}
\label{subsec:variations}

As in \cite{dosovitskiy2020image}, we observe that it is possible to modify the cross attention mechanism to further update features after the linear projection following attention computation. Moreover, it is also possible to project the input features to the space in which the [class] token lies within. We define the following variations:

\paragraph{Cross Attention with MLP}
The work of \cite{NIPS2017_3f5ee243} and \cite{dosovitskiy2020image} introduce a MLP or feedforward network to capture and process local patterns more globally. Thus we propose to add a MLP on top of Cross Attention, as Vision transformers:
% Regarding the architecture of transformers, we observe that following attention operation and the following projection, a feedforward network or MLP is used to further update the representation produced. To this end, we consider:
\begin{equation}
    \mbox{MLP}_\ell(\vq_{\ell}) = \mbox{GELU}(\vq_\ell W_{in}+b_{in})W_{out}+b_{out}.
    % \vq_{\ell+1} = W_\ell \cdot \ca_\ell(\vq_\ell, F_\ell),
    \label{eq:mlp_ca}
\end{equation}
Where the input and output dimensions remain the same and the inner layer has reduced dimension of $d_{in} = d_l\times 2$.\\

\paragraph{Projected Cross Attention}
On the operational level, our Cross Attention Block leverages the interactions between the [CLS] token and the features of a given model for a given layer \textit{l}, projecting to the dimension at the following stage \textit{l+1}. It is however possible to preserve the space in which this token lies, by the projection of the features at a given layer to the dimension of [CLS]
\begin{equation}
    % \mbox{CA}_\ell(Q, F_{\ell}) = \mbox{softmax}(\frac{Q_{\ell}(F_{\ell}W^K)^\top}{\sqrt{d_Q}})F_{\ell}W^V
    \ca_\ell(\vq_\ell, F_\ell) \defn (F_\ell W^V_\ell)\tran h_\ell(F_\ell W^K_\ell \vq_\ell)\in \real^{d_\ell}.
    % \ca_\ell(\vq_\ell, F_\ell) \defn F_\ell\tran \va = F_\ell\tran h_\ell(F_\ell \vq_\ell) \in \real^{d_\ell}.
    \label{eq:proj_ca}
\end{equation}
Where the projections are parameter matrices $W^K, W^V \in \real^{d_\ell\times d_Q}$.

On \autoref{sec:gen_ablation} we experiment with the different proposals for the cross attention mechanism and its integration into the CLS-Stream.

==> WACV_Backups/tex_wacv/figure_outdataset.tex <==
\begin{figure*}
\scriptsize
\centering
\setlength{\tabcolsep}{1.3pt}
%    \resizebox{\columnwidth}{!}{%
     \begin{tabular}{cccccccc}
           \mc{2}{Corridor}&\mc{2}{Greenhouse}&\mc{2}{Pool Inside}&\mc{2}{Wine Cellar}\\
           Input image&Raw Attention&Input image&Raw Attention&Input image&Raw Attention&Input image&Raw Attention\\
           \includegraphics[width=0.12\textwidth,height=0.08\textwidth]{Images/Outdataset/Corridor/Original/c1.jpg}&
           \includegraphics[width=0.12\textwidth,height=0.08\textwidth]{Images/Outdataset/Corridor/Attention/c1.jpg}&
           \includegraphics[width=0.12\textwidth,height=0.08\textwidth]{Images/Outdataset/Greenhouse/Original/celosie_02.jpg}&
           \includegraphics[width=0.12\textwidth,height=0.08\textwidth]{Images/Outdataset/Greenhouse/Attention/celosie_02.jpg}&
           \includegraphics[width=0.12\textwidth,height=0.08\textwidth]{Images/Outdataset/Poolinside/Original/003_1b.jpg}&
           \includegraphics[width=0.12\textwidth,height=0.08\textwidth]{Images/Outdataset/Poolinside/Attention/003_1b.jpg}&
           \includegraphics[width=0.12\textwidth,height=0.08\textwidth]{Images/Outdataset/WineCellar/Original/bodega2.jpg}&
           \includegraphics[width=0.12\textwidth,height=0.08\textwidth]{Images/Outdataset/WineCellar/Attention/bodega2.jpg}\\
           
           \includegraphics[width=0.12\textwidth,height=0.08\textwidth]{Images/Outdataset/Corridor/Original/1L_10_Corridor_A.jpg}&
           \includegraphics[width=0.12\textwidth,height=0.08\textwidth]{Images/Outdataset/Corridor/Attention/1L_10_Corridor_A.jpg}&
           \includegraphics[width=0.12\textwidth,height=0.08\textwidth]{Images/Outdataset/Greenhouse/Original/20070417klpcnatun_229_Ies_SCO.jpg}&
           \includegraphics[width=0.12\textwidth,height=0.08\textwidth]{Images/Outdataset/Greenhouse/Attention/20070417klpcnatun_229_Ies_SCO.jpg}&
           \includegraphics[width=0.12\textwidth,height=0.08\textwidth]{Images/Outdataset/Poolinside/Original/141821195_M.jpg}&
           \includegraphics[width=0.12\textwidth,height=0.08\textwidth]{Images/Outdataset/Poolinside/Attention/141821195_M.jpg}&
           \includegraphics[width=0.12\textwidth,height=0.08\textwidth]{Images/Outdataset/WineCellar/Original/bodega_45_18_yahoo.jpg}&
           \includegraphics[width=0.12\textwidth,height=0.08\textwidth]{Images/Outdataset/WineCellar/Attention/bodega_45_18_yahoo.jpg}\\
           
           \includegraphics[width=0.12\textwidth,height=0.08\textwidth]{Images/Outdataset/Corridor/Original/430_Korridor_300.jpg}&
           \includegraphics[width=0.12\textwidth,height=0.08\textwidth]{Images/Outdataset/Corridor/Attention/430_Korridor_300.jpg}&
           \includegraphics[width=0.12\textwidth,height=0.08\textwidth]{Images/Outdataset/Greenhouse/Original/20070418klpcnaecl_364_Ies_SCO.jpg}&
           \includegraphics[width=0.12\textwidth,height=0.08\textwidth]{Images/Outdataset/Greenhouse/Attention/20070418klpcnaecl_364_Ies_SCO.jpg}&
           \includegraphics[width=0.12\textwidth,height=0.08\textwidth]{Images/Outdataset/Poolinside/Original/catalogue_piscine_interieur.jpg}&
           \includegraphics[width=0.12\textwidth,height=0.08\textwidth]{Images/Outdataset/Poolinside/Attention/catalogue_piscine_interieur.jpg}&
           \includegraphics[width=0.12\textwidth,height=0.08\textwidth]{Images/Outdataset/WineCellar/Original/bodega_63_24_flickr.jpg}&
           \includegraphics[width=0.12\textwidth,height=0.08\textwidth]{Images/Outdataset/WineCellar/Attention/bodega_63_24_flickr.jpg}\\
           
           \includegraphics[width=0.12\textwidth,height=0.08\textwidth]{Images/Outdataset/Corridor/Original/06_Right_corridor_of_the_main_hall.jpg}&
           \includegraphics[width=0.12\textwidth,height=0.08\textwidth]{Images/Outdataset/Corridor/Attention/06_Right_corridor_of_the_main_hall.jpg}&
           \includegraphics[width=0.12\textwidth,height=0.08\textwidth]{Images/Outdataset/Greenhouse/Original/2026_2006_Grimm_s_Gardens_Greenhouse.jpg}&
           \includegraphics[width=0.12\textwidth,height=0.08\textwidth]{Images/Outdataset/Greenhouse/Attention/2026_2006_Grimm_s_Gardens_Greenhouse.jpg}&
           \includegraphics[width=0.12\textwidth,height=0.08\textwidth]{Images/Outdataset/Poolinside/Original/connolly_center_pool_inside_lg.jpg}&
           \includegraphics[width=0.12\textwidth,height=0.08\textwidth]{Images/Outdataset/Poolinside/Attention/connolly_center_pool_inside_lg.jpg}&
           \includegraphics[width=0.12\textwidth,height=0.08\textwidth]{Images/Outdataset/WineCellar/Original/bodega_78_08_flickr.jpg}&
           \includegraphics[width=0.12\textwidth,height=0.08\textwidth]{Images/Outdataset/WineCellar/Attention/bodega_78_08_flickr.jpg}\\              
    \end{tabular}
%    }
    \vspace{3pt}
    \caption{Raw attention maps obtained from our \Ours on images of the MIT 67 Scenes dataset~\cite{quattoni2009recognizing} on classes that do not exist in ImageNet. The network sees them at inference for the first time.}
    \label{fig:enter-label}
\end{figure*}

==> WACV_Backups/tex_wacv/figure_ra-passes.tex <==
\begin{figure*}[ht]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{cccccccc}
           \mr{2}{}&\mr{2}{\Th{Original}}&\mc{3}{\Th{First Pass}}&\mc{3}{\Th{Second Pass}}\\
            & &\gap-\Th{GC} & \ours-\Th{GC} & \ours-\Th{RA} &\gap-\Th{GC} & \ours-\Th{GC} & \ours-\Th{RA}\\
           {\rotatebox{90}{\small text}}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/Original/1019.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/F-Base-CAM/1019.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/F-Stream-CAM/1019.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/F-Stream-Raw/1019.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/S-Base-CAM/1019.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/S-Stream-CAM/1019.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/S-Stream-Raw/1019.jpeg}\\

           {\rotatebox{90}{\small text}}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/Original/274.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/F-Base-CAM/274.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/F-Stream-CAM/274.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/F-Stream-Raw/274.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/S-Base-CAM/274.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/S-Stream-CAM/274.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/S-Stream-Raw/274.jpeg}\\

           {\rotatebox{90}{\small text}}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/Original/963.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/F-Base-CAM/963.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/F-Stream-CAM/963.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/F-Stream-Raw/963.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/S-Base-CAM/963.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/S-Stream-CAM/963.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/S-Stream-Raw/963.jpeg}\\

           {\rotatebox{90}{\small text}}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/Original/1944.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/F-Base-CAM/1944.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/F-Stream-CAM/1944.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/F-Stream-Raw/1944.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/S-Base-CAM/1944.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/S-Stream-CAM/1944.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/S-Stream-Raw/1944.jpeg}\\         

          {\rotatebox{90}{\small text}}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/Original/711.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/F-Base-CAM/711.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/F-Stream-CAM/711.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/F-Stream-Raw/711.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/S-Base-CAM/711.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/S-Stream-CAM/711.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/S-Stream-Raw/711.jpeg}\\          
    \end{tabular}
    }
    \caption{\emph{Comparison between }}
    \label{fig:com_forwards}
\end{figure*}

==> WACV_Backups/tex_wacv/intro-1.tex <==
\section{Introduction}


%power of MHSA comes from : 1. weak inductive bias = more degrees of freedom
% 2. large context window help ? or not ?

%also less sensible to attacks of high frequency. MHSA smoothing ?


Since the re-popularization of deep learning in computer vision a decade ago, a large effort has been dedicated to finding efficient Neural Networks (NN) architectures.
While Convolutional NN (CNN) reigned supreme for a long time, the competition is now raising with Transformers.
Indeed CNNs apply a series of layers of convolutional filters, aggregate the spatial information while increasing the number of filters, resulting in dense global descriptors used for recognition.
Convolutions are particularly adequate to model image structure and there is no questioning about the great capabilities of such networks.
However, Transformers are bringing self-attention modules and new learning paradigms that can improve models further.

Self-attention layers are the key feature of Transformers. 
The input representation is projected into three matrices that are used to compute the attention map that is applied to the values matrix.
These modules allow higher order information to be diffused over the patches.
However, part of the information localization is lost on the way.

In this work, we aim at adapting self-attention and particularly the CLS \textcolor{green}{mechanism} into a CNN architecture.
We adopt a cross-attention module and build a stream to include attention information at several key stages of CNN. 
In the latest stage, our module replaces the global average pooling typically used to obtain attention-based pooling.

We propose to use our stream in a post-hoc interpretability scenario, meaning that we will use a fixed pre-trained network and aim to provide better interpretability using existing methods.
Moreover, our stream provides attention maps that can be used to understand what the networks attend to without any label relations.

More specifically we make the following contribution:
\begin{itemize}
    \item We propose a cross-attention module, derived from self-attention that focuses on the CLS aggregation.
    \item Our modules are built together in a stream that can connect and adapt to the layers of a CNN architecture.
    \item The trained stream helps explain a trained network, by providing an attention map independent of any categories, as well as improving the performance of existing post-hoc interpretability methods.
\end{itemize}

After a review of previous work, we present our method and experimental results.






==> WACV_Backups/tex_wacv/intro.tex <==
\section{Introduction}
\label{sec:intro}

Convolutional neural networks have had tremendous success in computer vision~\cite{he2016deep,liu2022convnet} but, due to their complexity, it is still an open problem how to explain or interpret their predictions. The most concrete achievement in this direction is to localize in an image what regions a prediction can be attributed to, by means of \emph{saliency maps}. \emph{Post-hoc} interpretability methods do so without changing the network architecture or training process and \emph{class activation mapping} (CAM)~\cite{zhou2016learning} has been a milestone in their development. CAM-based saliency maps are expressed as a linear combination of feature maps followed by an activation function and it is the definition of weights that determines different methods \cite{DBLP:journals/corr/SelvarajuDVCPB16,DBLP:journals/corr/abs-1710-11063,DBLP:journals/corr/abs-1910-01279}.
%Grad-CAM~\cite{DBLP:journals/corr/SelvarajuDVCPB16}, Grad-CAM++~\cite{DBLP:journals/corr/abs-1710-11063} and ScoreCAM~\cite{DBLP:journals/corr/abs-1910-01279}


Vision transformers~\cite{dosovitskiy2020image} are now strong competitors of convolutional networks, characterized by global interactions between patch embeddings in the form of \emph{self attention}. 
Based on a classification (\cls) token, their pooling mechanism allows localization by means of \emph{raw attention} maps. However, these maps are class agnostic, they can be of low quality~\cite{dino} and dedicated interpretability methods are required~\cite{chefer2021transformer}.

In this work, we make an important connection between CAM and the raw attention map of the \cls token. 
In particular, self attention is defined on all patch tokens, including \cls. Focusing on the cross attention between \cls and patch token embeddings, this is expressed as a collection of dot product similarities between embeddings, followed by softmax. 
We show that this collection of similarities is in fact a linear combination of feature maps, where the weights are the elements of the \cls token embedding. Hence, \textbf{the raw attention map of the \cls token has the same form as a class agnostic CAM-based saliency map}.

In addition, pooling in vision transformers is defined as a weighted average of patch token embeddings, where the weights are given by the raw attention map of the \cls token. This can be seen as reweighting, or soft masking, of the embeddings before \emph{global average pooling} (GAP). By contrast, pooling in convolutional networks is based on GAP only. We thus observe that \textbf{attention-based pooling is a form of masking in the feature space}. Masking, mostly in the input space, is common in interpretability methods~\cite{DBLP:journals/corr/abs-1910-01279} and their evaluation~\cite{DBLP:journals/corr/abs-1710-11063, petsiuk2018rise} to establish that a prediction is indeed due to a certain object of interest.

Motivated by the above observations, we design an attention-based pooling mechanism as a replacement for GAP in convolutional networks. Since this mechanism has the form of a CAM-based saliency map followed by masking, we aim to study the effect of this network modification in interpreting the network predictions.

Our pooling mechanism, called \emph{\OURS} (\emph{\Ours}), is implemented as a stream running in parallel with the backbone network. At different stages of the network, it allows interaction between a \cls token and patch embeddings by means of cross attention. The \cls token embedding is initialized as a learnable parameter and, at the output of the stream, provides a global image representation for classification.

We aim at post-hoc interpretability, therefore we keep the network and classifier frozen while learning the parameters of \Ours. We then obtain CAM-based saliency maps by existing post-hoc methods for both GAP and \Ours and compare their performance in terms of interpretability metrics as well as classification accuracy.

More specifically, we make the following contributions:
\begin{enumerate}[itemsep=2pt, parsep=0pt, topsep=3pt]
    \item We show that attention-based pooling in vision transformers is the same as soft masking by a class agnostic CAM-based saliency map (\autoref{subsec:motiv}).
    \item We design and inject an attention-based pooling mechanism into convolutional networks to replace GAP and study its effect on post-hoc interpretability (\autoref{subsec:CA-base}). This is a modification of the network but not of its training process.
    \item We show that this mechanism helps explain a trained network by improving the performance of existing post-hoc interpretability methods as well as providing a class agnostic raw attention map (\autoref{sec:exp}).
\end{enumerate}


==> WACV_Backups/tex_wacv/method-1.tex <==
\section{CLS-Pooling}
\begin{figure*}[t]
    \centering
    %\fig[0.45]{method}
    \includegraphics[scale=0.3]{Images/Method/Stream.pdf}
    \caption{Caption}
    \label{fig:fig_method}
\end{figure*}

\subsection{Preliminaries}
\begin{figure}[t]
    \centering
    %\fig[0.45]{method}
    \includegraphics[scale=0.3]{Images/Method/SelfAttention.pdf}
    \caption{Caption}
    \label{fig:fig_crossatt}
\end{figure}
In image classification, our objective is to classify an given image \textit{x}, with the most probable label \textit{y} from the category set $Y=\{y_1, y_2, \dots, y_n\}$. This is done by using an image classification model \textit{f} that can be trained in a supervised or self-supervised way.
\begin{equation}
    y = f(x)
\end{equation}
Assuming this model \textit{f} is made up from a sequence of operations (or layers), it is possible to dissect it at different depths \textit{k} and observe the representation $F_k$ of this given image in this space.
\begin{equation}
    F_k = f_k(F_{k-1})
\end{equation}
On another hand, it is feasible to make use of a classification token ({[class]}) \cite{DBLP:journals/corr/abs-1810-04805,DBLP:journals/corr/abs-2010-11929} that is used as an image representation to be used towards this task. In prior approaches, this token is prepended to the patch embedding of \textit{x}; whereas  in this approach, we aim at learning this representation by leveraging the interactions with feature maps at given points of a network. %Therefore, this token $Q$ is updated alongside \textit{F} at different depths of the network.

\subsection{Cross-Attention module}
Taking inspiration from \cite{DBLP:journals/corr/ChengDL16}; we devise a cross attention module (CA) that is built upon the sequential property of CNNs, to update a global image representation $Q$. To do so, in comparison to self attention; we compute the similarity between this representation and the feature maps for a given point. We preserve the scaling factor proposed in \cite{NIPS2017_3f5ee243} as the dimension of feature maps increases alongside depth; therefore the dimension of this representation is increased as well.
\begin{equation}
    \mbox{CA}_k(Q_{k}, F_{k+1}) = \mbox{softmax}(\frac{Q_{k}F^T_{k+1}}{\sqrt{dim_k}})F_{k+1}
\end{equation}
This class token is initialized with a normal distribution \ref{eq:qinit}, and is updated across given points in the network with the features found in the following stage. Conversely, as the feature maps width is increased alongside the depth of the network, we make use of a linear projection \textit{W} to allow our representation to interact with said features at different depths of \textit{f} \ref{eq:qklayer}.
% the width of our representation is increased via linear projection \textit{W} on top of the attention mechanism. %Our cross attention module is presented in figure \ref{fig:fig_crossatt}\\
\begin{equation}
    Q_0 \sim \mathcal{N}(1, 1) 
    \label{eq:qinit}
\end{equation}
\begin{equation}    
    Q_{k+1} = W_k(\mbox{CA}_{k}(Q_{k}, F_{k}))
    \label{eq:qklayer}
\end{equation}
Our Cross Attention model is summarized on figure \ref{fig:fig_crossatt}


\subsection{Cross-Attention Stream}
Taking into consideration this proposed attention module, we observe that it can be applied at different stages of \textit{f}. In particular, we focus on depths where changes in the area of feature maps gets reduced by pooling operations. Conversely, ever since its proposal GAP\cite{lin2013network} has been used to rely information from feature maps into the classifier stages for CNNs; however since this pooling approach is uniform, the representation observed by these operations does not completely convey the real contribution of certain image patches towards our classification task. To alleviate this, we utilize our {[class]} token to update the representation examined at earlier points in the model, while also pooling the features found in the latest convolutional block of \textit{f}. An example of this stream can be observed in figure \ref{fig:fig_method} where it is applied to a ResNet based architecture. 



==> WACV_Backups/tex_wacv/method-2.tex <==
\section{Method}

\subsection{Preliminaries}

\paragraph{Notation.}
Let $f: \cX \rightarrow \mathbb{R}^C$ denote a classifier network that maps an input image $\vx \in \cX$ to a logit vector $\vy= f(\vx) \in \mathbb{R}^C$, where $\cX$ is image space and $C$ is the number of classes. We denote the logit value of class $c$ as $y^c$ and obtain the corresponding probability by $p^c = \mbox{softmax}(\vy, c) \defn e^{y^c} / \sum_j e^{y^j}$.

\paragraph{CAM-based saliency maps.}
Assuming $f$ to be a CNN, a given layer $\ell$ and a class of interest $c$, we consider saliency maps given by the general formula
\begin{equation}
	S^c_\ell(\vx) \defn h \left( \sum_k w^c_k F^k_\ell \right),
\label{eq:sal}
\end{equation}
where $F^k_\ell$ denotes the activation map for the $k$-th channel, $w^c_k$ are weights defining a linear combination over channels and $h$ is an activation function. CAM~\citep{zhou2016learning} is defined for the last layer $L$ only with $h$ being the identity mapping and $w^c_k$ being the classifier weight connecting the $k$-th channel with class $c$. Grad-CAM~\citep{DBLP:journals/corr/SelvarajuDVCPB16} is defined for any layer $\ell$ with $h = \relu$ and weights
\begin{equation}
	w^c_k \defn \gap \left( \pder{y^c}{F^k_\ell} \right),
\label{eq:gcam}
\end{equation}
Where $\gap$ is global average pooling.

\paragraph{Self-Attention.}
Let $X \in \mathbb{R}^{s \times d}$ be the input of a self-attention module, where $d$ is the embedding dimension, and $s \defn w \times h + 1$ the patch size of width \textbf{\textit{w}} and height \textbf{\textit{h}} plus the [CLS] token. A self-attention module is defined as %  equals to the number of patches (with width \textit{w} and height \textit{h}) with the addition of the [CLS] token. 
\begin{equation}
    F_{\ell+1} \defn \mbox{softmax} \left( \frac{QK^{\top}}{\sqrt{d}} \right) V,
    \label{eq:self-attention}
\end{equation}
where $Q\defn W_Q X$, $K\defn W_K X$, $V\defn W_V X$ and $W_Q$, $W_K$, $W_V$ are learnable weights.\\

Ultimately, we observe that there is a similarity between the formulation of self attention and CAM methods, where if defined in a generic way it would be 
\begin{equation}
    S_\ell^C(x) \defn \mbox{NonLinearity}(\alpha\times F^k_\ell)
    \label{eq:CamIsAtt}
\end{equation}
We note that for CAM-based approaches the non-linearity utilized is ReLU; whereas for self attention, Softmax is used instead. On another hand, we observe that the calculation of the generic weighting coefficient $\alpha$ provides yet another difference; on self attention this is obtained by the matrix multiplication of $Q, K$ queries, whereas for CAM it is defined according to the specific approach being utilized.

\paragraph{Motivation.} 
[CLS] token~\citep{DBLP:journals/corr/abs-1810-04805,DBLP:journals/corr/abs-2010-11929} of self-attention is prepended to the patch embedding of $\vx$ and usually is used for classification as it gathers information from all patches according to self-attention. 
%Revisiting (\ref{eq:self-attention}), by only considering the [CLS] token $Q^{[CLS]} \in \mathbb{R}^{1\times d}$, we have $softmax(\frac{Q^{[CLS]} (W_KX)^{\top}}{\sqrt{d}})W_VX$, where $Q^{[CLS]}(W_KX)^{\top}$ calculates the similarity between global feature ($Q^{[CLS]}$) and local features of each patches ($W_KX$), then combines the local features ($W_VX$) according to this similarity vector. 
Revisiting (\ref{eq:self-attention}), if we only consider the [CLS] token $Q^{[CLS]} \in \mathbb{R}^{1\times d}$ as a global representation, we obtain
\begin{equation}
     F_{\ell+1}^{[CLS]} = \mbox{softmax}(\frac{Q^{[CLS]} (W_KX)^{\top}}{\sqrt{d}})W_VX
\end{equation}
where $Q^{[CLS]}(W_KX)^{\top}$ calculates the similarity between global feature ($Q^{[CLS]}$) and local features of each patches ($W_KX$), then $F_{\ell+1}^{[CLS]}$ is a linear combination of the local features ($W_VX$) according to this similarity vector. When $\ell + 1$ is the last layer, $F_{\ell+1}^{[CLS]}$ can be used for classification.

Convolutional neural networks are good at capturing local features but lack of insight of global information; thus we aim at learning this representation by leveraging interactions with feature maps at given points of a network, using a mechanism inspired from the self-attention operation to replace $\gap$
%and we use the mechanism which inspired from self-attention module to replace $\gap$.
   

\subsection{Cross-Attention Block}
\label{subsec:CA-base}
Inspired by the architecture of Transformers~\cite{NIPS2017_3f5ee243}, we devise a cross attention block (CA) that is built upon the sequential property of CNNs, to update a global image representation. For a given layer $\ell$, we denote it  as $Q_\ell \in \mathbb{R}^{1 \times d_\ell}$, where $d_\ell$ is the channel dimension of $F_\ell$. To do so, in comparison to self attention; we compute the similarity between this representation and the feature maps for a given point. We preserve the scaling factor proposed in \cite{NIPS2017_3f5ee243} as the dimension of feature maps increases alongside depth; therefore the dimension of this representation does as well.
\begin{equation}
    \mbox{CA}_\ell(Q_{\ell}, F_{\ell}) = \mbox{softmax}(\frac{Q_{\ell}F^\top_{\ell}}{\sqrt{d_\ell}})F_{\ell}
    \label{eq:CA-base}
\end{equation}
This class token is initialized with a normal distribution (\ref{eq:qinit}), and is updated across given points in the network with the features found in the following stage. Conversely, as the feature maps width is increased alongside the depth of the network, we make use of a linear projection $\vw_\ell$ (\ref{eq:qklayer}) as to allow our representation to interact with said features at different layers of the network. 
% the width of our representation is increased via linear projection \textit{W} on top of the attention mechanism. %Our cross attention module is presented in Figure \ref{fig:fig_crossatt}\\

\begin{equation}
    Q_0 \sim \mathcal{N}(1, 1) 
    \label{eq:qinit}
\end{equation}
\begin{equation}    
    Q_{\ell+1} = \vw_\ell(\mbox{CA}_{\ell}(Q_{\ell}, F_{\ell}))
    \label{eq:qklayer}
\end{equation}
Our base Cross Attention Block is summarized on Figure \ref{fig:fig_crossatt}%\autoref{fig:fig_crossatt}


\begin{figure}[t]
    \centering
    \begin{tikzpicture}
        \node (Q) at (4.5, -0.5) {Q$_\ell$};
        % \node (dimq) at (5, 0) {\scriptsize${1\times d_\ell}$};
        \node (F) at (2.5, -0.5) {F$_{\ell}$};
        % \node (dimft) at (3.0, -0) {\scriptsize${d_{\ell}\times p}$};
        \node (empt1) at (1.75, -0.5) {};
        \node[shape=circle,draw=black] (mm1) at (3.5, 0.5) {$\times$};
        % \node (dimraw) at (4,1) {\scriptsize$1\times p$};
        \node[shape=rectangle,draw=black](scale) at (3.5, 1.5) {scale};
        % \node (dimf) at (2.5, 3.175) {\scriptsize${p\times d_{\ell}}$};
        \node (soft) at (4.125, 2.25) {\footnotesize softmax};
        \node[shape=circle,draw=black] (mm2) at (3.5, 3) {$\times$};
        % \node[shape=rectangle,draw=black](project) at (3.5, 4) {$w_l: d_\ell\times d_{\ell+1}$ };
        \node[shape=rectangle,draw=black](project) at (3.5, 4) {$w_l$};
        % \node (dimscaled) [] at (4.25, 3.5) {\scriptsize $1\times d_\ell$};
        % \node [shape=circle,draw=black](sum1) at (3.5, 4) {+};
        % \node [shape=rectangle,draw=black](norm) at (3.5, 5.75) {LayerNorm};
        \node (Qplus1) at (3.5, 5.25) {Q$_{\ell+1}$};
        % \node (dimql) [align=left] at (4.25, 4.75) {\scriptsize$1\times d_{\ell+1}$};
        % \node (empt2) at (5.75, -0.5) {};
        
        \draw[->] (Q) |- node {} (mm1);
        \draw[->] (F) |- node {} (mm1);
        % \draw[-] (Q) -| node {} (empt2);
        % \draw[->] (empt2.center) |- node {} (sum1);
        \draw[->] (mm1) -- node {} (scale);
        \draw[->] (scale) -- node {} (mm2);
        \draw[-] (F) -| node {} (empt1.center);
        \draw[->] (empt1.center) |- node {} (mm2);
        \draw[->] (mm2) -- node {} (project);
        % \draw[->] (sum1) -- node {} (project);
        \draw[->] (project) -- node {} (Qplus1);
        % \draw[->] (norm) -- node {} (Qplus1);
    \end{tikzpicture}
    \caption{A Cross Attention Block. We denote matrix multiplication as "$\otimes$". The softmax operation is performed on each row). For a given layer $\ell$ we update our [CLS] token $Q_\ell$; by computing its scaled cross attention with the feature maps $F_\ell$, that are then projected to the channel dimension in the following stage, using a dense layer parametrized by $w_\ell$.}
    \label{fig:fig_crossatt}
\end{figure}

\subsection{Variations}
\label{subsec:variations}
Next we describe several versions of the Cross Attention Block.\\
\begin{figure*}[t]
    \centering
    \begin{tikzpicture}[font={\tiny},]   
         %% CNN branch
        \node(input) at (-5.5, 0) {\includegraphics[width=.1\textwidth]{Images/Method/input.jpg}};
        \node[] at (input.north) {\footnotesize Input image $\vx$};
        \node[draw, trapezium, rotate=-90,trapezium angle=75, align=center] (res0) at (-3.5,0) {\rotatebox{90}{\parbox{1.0cm}{\centering{\footnotesize Res-0}\\$d_\ell:$\\64}}};
        \node[draw, trapezium, rotate=-90,trapezium angle=75, align=center] (res1) at (-1.5,0) {\rotatebox{90}{\parbox{1.0cm}{\centering{\footnotesize Res-1}\\$d_\ell:$\\64*BE}}};
        \node[draw, trapezium, rotate=-90,trapezium angle=75, align=center] (res2) at (0.5,0) {\rotatebox{90}{\parbox{1.0cm}{\centering{\footnotesize Res-2}\\$d_\ell:$\\128*BE}}};
        \node[draw, trapezium, rotate=-90,trapezium angle=75, align=center] (res3) at (2.5,0) {\rotatebox{90}{\parbox{1.0cm}{\centering{\footnotesize Res-3}\\$d_\ell:$\\256*BE}}};
        \node[draw, trapezium, rotate=-90,trapezium angle=75, align=center] (res4) at (4.5,0) {\rotatebox{90}{\parbox{1.0cm}{\centering{\footnotesize Res-4}\\$d_\ell:$\\512*BE}}};
        \node[](empt1) at (6.5, 0){};
        \node[draw, rotate=90, align=center] (class) at (7,0) {\footnotesize Classifier};
        \node(logit) at (7.75, 0) {\small$\vy$};
        %%% CLS stream
        \node[align=center](clsin) at (-4, -1.5) {{\footnotesize[CLS],}\\$d_\ell: 64$};
        \node[draw, align=center](CA0) at (-2.5, -1.5) {{\footnotesize CA-0}, \\$d_\ell:$\\64*BE};
        \node[draw, align=center](CA1) at (-0.5, -1.5) {{\footnotesize CA-1}, \\$d_\ell:$\\128*BE};
        \node[draw, align=center](CA2) at (1.5, -1.5) {{\footnotesize CA-2}, \\$d_\ell:$\\256*BE};
        \node[draw, align=center](CA3) at (3.5, -1.5) {{\footnotesize CA-3}, \\$d_\ell:$\\512*BE};
        \node[draw, align=center](CA4) at (5.5, -1.5) {{\footnotesize CA-4}, \\$d_\ell:$\\512*BE};

        %% CNN backbone
        \node(empt0) at (-4.65, 0) {};
        \draw[->] (empt0.center) -- node {} (res0);
        \draw[->] (res0) -- node {} (res1);
        \draw[->] (res1) -- node {} (res2);
        \draw[->] (res2) -- node {} (res3);
        \draw[->] (res3) -- node {} (res4);
        \draw[->] (res1) -- node {} (res2);
        \draw[->] (res2) -- node {} (res3);
        \draw[->] (res3) -- node {} (res4);
        \draw[->, blue, dashed] (res4) -- node {\blue{\normalsize//}} (class);
        \node[](GAP) at (6,0.25) {\footnotesize\blue{$\gap$}};
        \draw[->] (class) -- node {} (logit);
        %% CLS Stream
        \draw[->] (clsin) -- node {} (CA0);
        \draw[dashed, ->] (res0.north) -|node {} (CA0);
        \draw[->] (CA0) -- node {} (CA1);
        \draw[dashed, ->] (res1.north) -|node {} (CA1);
        \draw[->] (CA1) -- node {} (CA2);
        \draw[dashed, ->] (res2.north) -|node {} (CA2);
        \draw[->] (CA2) -- node {} (CA3);
        \draw[dashed, ->] (res3.north) -|node {} (CA3);
        \draw[->] (CA3) -- node {} (CA4);
        \draw[dashed, ->] (res4.north) -|node {} (CA4);
        \draw[-] (CA4.east) -| node {} (empt1.center);
        \draw[->] (empt1.center) -- node {} (class);        
        % \path[->] (CA4.east) edge[bend right,left] node {} (class.north);
        % \path [->] (B) edge[bend right=60] node {$1$} (E); 
    \end{tikzpicture}
    \caption{Cross Attention Stream applied to ResNet-based architectures. Given a CNN backbone $f(\cdot)$, we replace global average pooling with  the introduction of a global representation [CLS] learned with the inclusion of the cross attention attention stream.}
    \label{fig:fig_method}
\end{figure*}

\noindent\textbf{Cross Attention with MLP}
Regarding the architecture of transformers, we observe that following attention operation and the following projection, a feedforward network or MLP is used to further update the representation produced. To this end, we consider:\\
\begin{equation}
    \mbox{MLP}(x) = GELU(xW_1+b_1)W_2+b_2
\end{equation}
Where we maintain input and output dimensions, while the inner layer presents dimension $d_{inner} = d_l\times 2$.\\

\noindent\textbf{Projected Cross Attention}
On the operational level, our Cross Attention Block leverages the interactions between the [CLS] token and the features of a given model for a given layer \textit{l}, projecting to the dimension at the following stage \textit{l+1}. It is however possible to preserve the space in which this token lies, by the projection of the features at a given layer to the dimension of [CLS]
\begin{equation}
    \mbox{CA}_\ell(Q, F_{\ell}) = \mbox{softmax}(\frac{Q_{\ell}(F_{\ell}W^K)^\top}{\sqrt{d_Q}})F_{\ell}W^V
\end{equation}
Where the projections are parameter matrices $W^K, W^V \in \mathbb{R}^{d_\ell\times d_Q}$.

Based on these modifications for the Cross-Attention Block, we opt to keep our approach as simple as possible by using the base approach without extra projections nor MLP; nevertheless, we demonstrate the differences in performance when we choose any of the proposed variations of the self attention, as shown on Table \ref{tab:CA_variations}
 
\subsection{CLS Stream}
\noindent Taking into consideration this proposed attention module, we observe that it can be applied at different blocks of \textit{f}. In particular, we focus on depths where critical operations take place for a given network (\ie in between residual layers for ResNet architectures). Conversely, ever since its proposal GAP has been used to rely information from feature maps into the classifier stages for CNNs; however since this pooling approach is uniform, the contribution of relevant image patches towards classification is reduced. To alleviate this, we utilize our {[class]} token to update the representation examined at earlier points in the model, while also pooling the features found in the latest convolutional block of \textit{f}. An example of this stream can be observed in Figure \ref{fig:fig_method} where it is applied to a ResNet based architecture.
%Taking into consideration this proposed attention module, we observe that it can be applied at different blocks of \textit{f}. In particular, we focus on depths where changes in the area of feature maps gets reduced by pooling operations. Conversely, ever since its proposal GAP has been used to rely information from feature maps into the classifier stages for CNNs; however since this pooling approach is uniform, the contribution of relevant image patches towards classification is reduced. To alleviate this, we utilize our {[class]} token to update the representation examined at earlier points in the model, while also pooling the features found in the latest convolutional block of \textit{f}. An example of this stream can be observed in Figure \ref{fig:fig_method} where it is applied to a ResNet based architecture. 


%% To do: v3 without FC and Matrix V3 FC, no FC

==> WACV_Backups/tex_wacv/method-3.tex <==
\section{Method}

%------------------------------------------------------------------------------
\input{tex/mainfig}
%------------------------------------------------------------------------------

\subsection{Preliminaries and background}
\label{subsec:prelim}

\paragraph{Notation}

Let $f: \cX \rightarrow \real^C$ be a classifier network that maps an input image $\vx \in \cX$ to a logit vector $\vy= f(\vx) \in \real^C$, where $\cX$ is image space and $C$ is the number of classes. A class probability vector is obtained by $\vp = \softmax(\vy)$. The logit and probability of class $c$ are denoted by
$y^c$ and $p^c = \softmax(\vy)^c \defn e^{y^c} / \sum_j e^{y^j}$, respectively. Let $\vF_\ell \in \real^{w_\ell \times h_\ell \times d_\ell}$ be the feature tensor at layer $\ell$ of the network, where $w_\ell \times h_\ell$ is the spatial resolution and $d_\ell$ the embedding dimension, or number of channels. The feature map of channel $k$ is denoted by $F^k_\ell \in \real^{w_\ell \times h_\ell}$. By $\ell$ we may refer to an arbitrary layer of $f$ or a larger compositional block, \eg, a stage.

\paragraph{CAM-based saliency maps}

Given a class of interest $c$ and a layer $\ell$, we consider the saliency maps $S^c_\ell \in \real^{w_\ell \times h_\ell}$ given by the general formula
\begin{equation}
	S^c_\ell \defn h \left( \sum_k \alpha^c_k F^k_\ell \right),
\label{eq:sal}
\end{equation}
where $\alpha^c_k$ are weights defining a linear combination over channels and $h$ is an activation function. Assuming \emph{global average pooling} (GAP) of the last feature tensor $\vF_L$ followed by a linear classifier, CAM~\citep{zhou2016learning} is defined for the last layer $L$ only, with $h$ being the identity mapping and $\alpha^c_k$ the classifier weight connecting channel $k$ with class $c$. Grad-CAM~\citep{DBLP:journals/corr/SelvarajuDVCPB16} is a generalization of CAM defined for any architecture and layer $\ell$, with $h = \relu$ and weights
\begin{equation}
	\alpha^c_k \defn \gap \left( \pder{y^c}{F^k_\ell} \right).
\label{eq:gcam}
\end{equation}
% The \cls token is used for classification as it gathers information from all patches according to self-attention.

%------------------------------------------------------------------------------

\paragraph{Self-Attention}

Let $X_\ell \in \real^{t_\ell \times d_\ell}$ denote the sequence of token embeddings of a vision transformer~\cite{dosovitskiy2020image} at layer $\ell$, where $t_\ell \defn w_\ell h_\ell + 1$ is the number of tokens, including patch tokens and the \cls token, and $d_\ell$ is the embedding dimension. The \emph{query}, \emph{key} and \emph{value} matrices are defined as $Q = X_\ell W_Q$, $K = X_\ell W_K$, $V = X_\ell W_V \in \real^{t_\ell \times d_\ell}$, where $W_Q, W_K, W_V \in \real^{d_\ell \times d_\ell}$ are learnable linear projections. The \emph{attention matrix} $A \in \real^{t_\ell \times t_\ell}$ expresses pairwise dot-product similarities between queries (rows of $Q$) and keys (rows of $K$), normalized by softmax over rows
\begin{equation}
	A = \softmax \left( \frac{Q K\tran}{\sqrt{d_\ell}} \right).
\label{eq:attention}
\end{equation}
For each token, the \emph{self-attention} operation is then defined as an average of all values (rows of $V$) weighted by attention (the corresponding  row of $A$),
\begin{equation}
	\sa(X_\ell) \defn A V \in \real^{t_\ell \times d_\ell}.
\label{eq:SA}
\end{equation}
At the last layer $L$, the \cls token embedding is used as a global image representation for classification as it gathers information from all patches by weighted averaging, replacing \gap. Thus, at the last layer, it is only cross attention between \cls and the patch tokens that matters.

%------------------------------------------------------------------------------

\subsection{Motivation}
\label{subsec:motiv}

\paragraph{Cross attention}

Let matrix $F_\ell \in \real^{p_\ell \times d_\ell}$ be a reshaping of feature tensor $\vF_\ell$ at layer $\ell$, where $p_\ell \defn w_\ell h_\ell$ is the number of patch tokens without \cls, and let $\vq_\ell \in \real^{d_\ell}$ be the \cls token embedding at layer $\ell$. By focusing on the \emph{cross attention} only between the \cls (query) token $\vq_\ell$ and the patch (key) tokens $F_\ell$ and by ignoring projections $W_Q, W_K, W_V$ for simplicity, attention $A$~\eq{attention} is now a $1 \times p_\ell$ matrix that can be written as a vector $\va \in \real^{p_\ell}$
\begin{equation}
	\va = A\tran = \softmax \left( \frac{F_\ell \vq_\ell}{\sqrt{d_\ell}} \right).
\label{eq:cross-attention}
\end{equation}
Here, $F_\ell \vq_\ell$ expresses the pairwise similarities between the global \cls feature $\vq_\ell$ and the local patch features $F_\ell$. Now, by replacing $\vq_\ell$ by an arbitrary vector $\valpha \in \real^{d_\ell}$ and by writing the feature matrix as
$F_\ell = (\vf_\ell^1 \dots \vf_\ell^{d_\ell})$ where $\vf_\ell^k = \vect(F_\ell^k) \in \real^{p_\ell}$ for channel $k$, attention \eq{cross-attention} becomes
\begin{equation}
	\va = h_\ell (F_\ell \valpha) =
		h_\ell \left( \sum_k \alpha_k \vf_\ell^k \right).
\label{eq:connection}
\end{equation}
This takes the same form as~\eq{sal}, with feature maps $F_\ell^k$ being vectorized into $\vf_\ell^k$ and the nonlinearity is defined as $h_\ell(\vx) = \softmax(\vx / \sqrt{d_\ell})$. We thus observe the following.

\begin{quote}
	\emph{Pairwise similarities between one query and all patch token embeddings in cross attention are the same as a linear combination of feature maps in CAM-based saliency maps, where the weights are determined by the elements of the query.}
\end{quote}

As it stands, one difference between~\eq{sal} and~\eq{connection} is that~\eq{connection} is class agnostic, although it could be extended by using one query (weight) vector per class. For simplicity, we choose the class agnostic form  in the sequel. We also choose to have no query/key/value projections. We do experiment with extended versions in \autoref{sec:gen_ablation}.

\paragraph{Pooling, or masking}

We are thus motivated to integrate an attention mechanism into any network such that making a prediction and explaining (localizing) it are inherently connected. In particular, considering cross attention only between \cls and patch tokens~\eq{cross-attention}, equation~\eq{SA} becomes
\begin{align}
	\ca_\ell(\vq_\ell, F_\ell) \defn F_\ell\tran \va = F_\ell\tran h_\ell(F_\ell \vq_\ell) \in \real^{d_\ell}.
\label{eq:CA}
\end{align}
This is a weighted average of the local patch features $F_\ell$ with attention vector $\va$ expressing the weights. It can be used as a global image representation, replacing \gap.

Now, considering that $\va$ is obtained exactly as CAM-based saliency maps~\eq{connection}, we can think of the weighted averaging operation as \emph{soft masking}, similarly to occlusion (masking)-based methods~\citep{petsiuk2018rise,fong2017interpretable,fong2019understanding,schulz2020restricting,ribeiro2016should,DBLP:journals/corr/abs-1910-01279,zhang2023opti} and certain evaluation metrics~\cite{petsiuk2018rise}. It takes place in the feature space, whereas for interpretability it is common to mask in the input space. Masking in feature space is much more efficient as requires only one forward and has been explored for interpretability too~\cite{schulz2020restricting}.

%------------------------------------------------------------------------------

\subsection{Cross attention stream}
\label{subsec:CA-base}

We thus design a \emph{cross attention stream} (\Ours), which is a processing stream placed in parallel with any network $f$, interacting with image features at given points of $f$, using a cross attention mechanism to replace $\gap$. An example is shown in \autoref{fig:fig_method}, applied to a ResNet-based architecture.

In general, we use a classification token embedding to build a global image representation along the stream. It is initialized as a learnable parameter $\vq_0 \in \real^{d_0}$, and it is updated by interacting with local image features at points between blocks of $f$ where critical operations take place, such as change of spatial resolution or embedding dimension, \eg between stages for ResNet. In particular, we decompose $f$ as
\begin{equation}
	f = f_0 \circ \dots \circ f_L \circ \gap \circ g
\label{eq:f-decomp}
\end{equation}
such that features $F_\ell \in \real^{p_\ell \times d_\ell}$ of layer (stage) $\ell$ are initialized as $F_{-1} = \vx$ and updated according to
\begin{equation}
	F_\ell = f_\ell(F_{\ell-1})
\label{eq:f-layer}
\end{equation}
for $0 \le \ell \le L$. The last layer features $F_L$ are followed by $\gap$ and $g: \real^{d_L} \to \real^C$ is the classifier, mapping to the logit vector $\vy$. As in \autoref{subsec:motiv}, $p_\ell$ is the number of patch tokens and $d_\ell$ the embedding dimension of stage $\ell$.

In parallel, the sequence of classification token embeddings $\vq_\ell \in \real^{d_\ell}$ along the stream interacts with $F_\ell$ at each stage $\ell$. Referring to the global representation $\vq_\ell$ as \emph{query} or \cls and to the local image features $F_\ell$ as \emph{key} or patch embeddings, the interaction consists of cross attention followed by a linear projection $W_\ell \in \real^{d_{\ell+1} \times d_\ell}$ to account for changes of embedding dimension between the corresponding stages of $f$:
\begin{equation}
	\vq_{\ell+1} = W_\ell \cdot \ca_\ell(\vq_\ell, F_\ell),
\label{eq:qk-layer}
\end{equation}
for $0 \le \ell \le L$, where \ca is defined as in~\eq{CA}.

Image features $F_0, \dots, F_L$ do not change by injecting our \Ours into network $f$. However, the final global image representation and hence the prediction do change. In particular, at the last stage $L$, $\vq_{L+1}$ is used as a global image representation for classification, replacing \gap over $F_L$. The final prediction is $g(\vq_{L+1}) \in \real^C$. Unlike \gap, the weights of different image patches in the linear combination are non-uniform, enhancing the contribution of relevant patches in the prediction.


==> WACV_Backups/tex_wacv/method.tex <==
\section{Method}

%------------------------------------------------------------------------------
\begin{figure*}[t]
\centering
% editable at https://docs.google.com/drawings/d/1nfqVV_dNqSV9g5UBuNopPLvubcEZx-vvg4K0ZCvNdfU/edit
\fig[.7]{Images/CA-CAM/CA-CAM}
\vspace{3pt}
\caption{\emph{Visualization of eq.~\eq{connection}.} On the left, a feature tensor $\vF \in \real^{w \times h \times d}$ is multiplied by the vector $\valpha \in \real^d$ in the channel dimension, like in $1 \times 1$ convolution, where $w \times h$ is the spatial resolution and $d$ is the number of channels. This is \emph{cross attention} (CA)~\cite{dosovitskiy2020image} between the query $\valpha$ and the key $\vF$. On the right, a linear combination of feature maps $F^1, \dots, F^d \in \real^{w \times h}$ is taken with weights $\alpha_1, \dots, \alpha_d$. This is a \emph{class activation mapping} (CAM)~\cite{zhou2016learning} with class agnostic weights. Eq.~\eq{connection} expresses the fact that these two quantities are the same, provided that $\valpha = (\alpha_1, \dots, \alpha_d)$ and $\vF$ is reshaped as $F = (\vf^1 \dots \vf^d) \in \real^{p \times d}$, where $p = wh$ and $\vf^k = \vect(F^k) \in \real^{p}$ is the vectorized feature map of channel $k$.}
\label{fig:connection}
\end{figure*}
%------------------------------------------------------------------------------

\subsection{Preliminaries and background}
\label{subsec:prelim}

\paragraph{Notation}

Let $f: \cX \rightarrow \real^C$ be a classifier network that maps an input image $\vx \in \cX$ to a logit vector $\vy= f(\vx) \in \real^C$, where $\cX$ is the image space and $C$ is the number of classes. A class probability vector is obtained by $\vp = \softmax(\vy)$. The logit and probability of class $c$ are respectively denoted by $y^c$ and $p^c = \softmax(\vy)^c \defn e^{y^c} / \sum_j e^{y^j}$. Let $\vF_\ell \in \real^{w_\ell \times h_\ell \times d_\ell}$ be the feature tensor at layer $\ell$ of the network, where $w_\ell \times h_\ell$ is the spatial resolution and $d_\ell$ the embedding dimension, or number of channels. The feature map of channel $k$ is denoted by $F^k_\ell \in \real^{w_\ell \times h_\ell}$. By $\ell$ we may refer to an arbitrary layer of $f$ or a larger compositional block, \eg, a stage.

\paragraph{CAM-based saliency maps}

Given a class of interest $c$ and a layer $\ell$, we consider the saliency maps $S^c_\ell \in \real^{w_\ell \times h_\ell}$ given by the general formula
\begin{equation}
	S^c_\ell \defn h \left( \sum_k \alpha^c_k F^k_\ell \right),
\label{eq:sal}
\end{equation}
where $\alpha^c_k$ are weights defining a linear combination over channels and $h$ is an activation function. Assuming \emph{global average pooling} (GAP) of the last feature tensor $\vF_L$ followed by a linear classifier, CAM~\citep{zhou2016learning} is defined for the last layer $L$ only, with $h$ being the identity mapping and $\alpha^c_k$ the classifier weight connecting channel $k$ with class $c$. Grad-CAM~\citep{DBLP:journals/corr/SelvarajuDVCPB16} is a generalization of CAM defined for any architecture and layer $\ell$, with $h = \relu$ and weights
\begin{equation}
	\alpha^c_k \defn \gap \left( \pder{y^c}{F^k_\ell} \right).
\label{eq:gcam}
\end{equation}

%------------------------------------------------------------------------------

\paragraph{Self-Attention}

Let $X_\ell \in \real^{t_\ell \times d_\ell}$ denote the sequence of token embeddings of a vision transformer~\cite{dosovitskiy2020image} at layer $\ell$, where $t_\ell \defn w_\ell h_\ell + 1$ is the number of tokens, including patch tokens and the \cls token, and $d_\ell$ is the embedding dimension. The \emph{query}, \emph{key} and \emph{value} matrices are defined as $Q = X_\ell W_Q$, $K = X_\ell W_K$, $V = X_\ell W_V \in \real^{t_\ell \times d_\ell}$, where $W_Q, W_K, W_V \in \real^{d_\ell \times d_\ell}$ are learnable linear projections. The \emph{attention matrix} $A \in \real^{t_\ell \times t_\ell}$ expresses pairwise dot-product similarities between queries (rows of $Q$) and keys (rows of $K$), normalized by softmax over rows
\begin{equation}
	A = \softmax \left( \frac{Q K\tran}{\sqrt{d_\ell}} \right).
\label{eq:attention}
\end{equation}
For each token, the \emph{self-attention} operation is then defined as an average of all values (rows of $V$) weighted by attention (the corresponding  row of $A$),
\begin{equation}
	\sa(X_\ell) \defn A V \in \real^{t_\ell \times d_\ell}.
\label{eq:SA}
\end{equation}
At the last layer $L$, the \cls token embedding is used as a global image representation for classification as it gathers information from all patches by weighted averaging, replacing \gap. Thus, at the last layer, it is only cross attention between \cls and the patch tokens that matters.



\subsection{Motivation}
\label{subsec:motiv}

\paragraph{Cross attention}

Let matrix $F_\ell \in \real^{p_\ell \times d_\ell}$ be a reshaping of feature tensor $\vF_\ell$ at layer $\ell$, where $p_\ell \defn w_\ell h_\ell$ is the number of patch tokens without \cls, and let $\vq_\ell \in \real^{d_\ell}$ be the \cls token embedding at layer $\ell$. By focusing on the \emph{cross attention} only between the \cls (query) token $\vq_\ell$ and the patch (key) tokens $F_\ell$ and by ignoring projections $W_Q, W_K, W_V$ for simplicity, attention $A$~\eq{attention} is now a $1 \times p_\ell$ matrix that can be written as a vector $\va \in \real^{p_\ell}$
\begin{equation}
	\va = A\tran = \softmax \left( \frac{F_\ell \vq_\ell}{\sqrt{d_\ell}} \right).
\label{eq:cross-attention}
\end{equation}
Here, $F_\ell \vq_\ell$ expresses the pairwise similarities between the global \cls feature $\vq_\ell$ and the local patch features $F_\ell$. Now, by replacing $\vq_\ell$ by an arbitrary vector $\valpha \in \real^{d_\ell}$ and by writing the feature matrix as $F_\ell = (\vf_\ell^1 \dots \vf_\ell^{d_\ell})$ where $\vf_\ell^k = \vect(F_\ell^k) \in \real^{p_\ell}$ for channel $k$, attention \eq{cross-attention} becomes
\begin{equation}
	\va = h_\ell (F_\ell \valpha) =
		h_\ell \left( \sum_k \alpha_k \vf_\ell^k \right).
\label{eq:connection}
\end{equation}
This takes the same form as~\eq{sal}, with feature maps $F_\ell^k$ being vectorized into $\vf_\ell^k$ and the activation function is defined as $h_\ell(\vx) = \softmax(\vx / \sqrt{d_\ell})$. Eq.~\eq{connection} is visualized in \autoref{fig:connection}. We thus observe the following.

\begin{quote}
	\emph{Pairwise similarities between one query and all patch token embeddings in cross attention are the same as a linear combination of feature maps in CAM-based saliency maps, where the weights are determined by the elements of the query.}
\end{quote}

As it stands, one difference between~\eq{sal} and~\eq{connection} is that~\eq{connection} is class agnostic, although it could be extended by using one query (weight) vector per class. For simplicity, we choose the class agnostic form in the following. We also choose to have no query/key projections. However, we do provide additional experiments with class specific representation as well as projections in \autoref{sec:gen_ablation}. 

\paragraph{Pooling, or masking}

We are thus motivated to integrate an attention mechanism into any network such that making a prediction and explaining (localizing) it are inherently connected. In particular, considering cross attention only between \cls and patch tokens~\eq{cross-attention}, equation~\eq{SA} becomes
\begin{align}
	\ca_\ell(\vq_\ell, F_\ell) \defn F_\ell\tran \va = F_\ell\tran h_\ell(F_\ell \vq_\ell) \in \real^{d_\ell}.
\label{eq:CA}
\end{align}
By writing the transpose of feature matrix as $F_\ell\tran = (\vphi_\ell^1 \dots \vphi_\ell^{p_\ell})$ where $\vphi_\ell^i \in \real^{d_\ell}$ is the feature of patch $i$, this is a weighted average of the local patch features $F_\ell\tran$ with attention vector $\va = (a_1, \dots, a_{p_\ell})$ expressing the weights:
\begin{align}
	\ca_\ell(\vq_\ell, F_\ell) \defn F_\ell\tran \va = \sum_i a_i \vphi_\ell^i.
\label{eq:CA-gap}
\end{align}
We can think of it as as feature \emph{reweighting} or \emph{soft masking} in the feature space, followed by \gap.

Now, considering that $\va$ is obtained exactly as CAM-based saliency maps~\eq{connection}, this operation is similar to occlusion (masking)-based methods~\citep{petsiuk2018rise, fong2017interpretable, fong2019understanding, schulz2020restricting, ribeiro2016should,DBLP:journals/corr/abs-1910-01279, zhang2023opti} and evaluation metrics~\cite{DBLP:journals/corr/abs-1710-11063, petsiuk2018rise}, where a CAM-based saliency map is commonly used to mask the input image. We thus observe the following.

\begin{quote}
	\emph{Attention-based pooling is a form of feature reweighting or soft masking in the feature space followed by \gap, where the weights are given by a class agnostic CAM-based saliency map.}
\end{quote}


%------------------------------------------------------------------------------

\subsection{Cross attention stream}
\label{subsec:CA-base}

Motivated by the observations above, we design a \emph{\OURS} (\emph{\Ours}) in parallel to any network. It takes input features at key locations of the network and uses cross attention to build a global image representation and replace $\gap$ before the classifier. An example is shown in \autoref{fig:fig_method}, applied to a ResNet-based architecture.

\paragraph{Architecture}

More formally, given a network $f$, we consider points between blocks of $f$ where critical operations take place, such as change of spatial resolution or embedding dimension, \eg between stages for ResNet. We decompose $f$ at these points as
\begin{equation}
	f = g \circ \gap \circ f_L \circ \dots \circ f_0
\label{eq:f-decomp}
\end{equation}
such that features $F_\ell \in \real^{p_\ell \times d_\ell}$ of layer (stage) $\ell$ are initialized as $F_{-1} = \vx$ and updated according to
\begin{equation}
	F_\ell = f_\ell(F_{\ell-1})
\label{eq:f-layer}
\end{equation}
for $0 \le \ell \le L$. The last layer features $F_L$ are followed by \gap and $g: \real^{d_L} \to \real^C$ is the classifier, mapping to the logit vector $\vy$. As in \autoref{subsec:motiv}, $p_\ell$ is the number of patch tokens and $d_\ell$ the embedding dimension of stage $\ell$.

In parallel, we initialize a classification token embedding as a learnable parameter $\vq_0 \in \real^{d_0}$ and we build a sequence of updated embeddings $\vq_\ell \in \real^{d_\ell}$ along a stream that interacts with $F_\ell$ at each stage $\ell$. Referring to the global representation $\vq_\ell$ as \emph{query} or \cls and to the local image features $F_\ell$ as \emph{key} or patch embeddings, the interaction consists of cross attention followed by a linear projection $W_\ell \in \real^{d_{\ell+1} \times d_\ell}$ to account for changes of embedding dimension between the corresponding stages of $f$:
\begin{equation}
	\vq_{\ell+1} = W_\ell \cdot \ca_\ell(\vq_\ell, F_\ell),
\label{eq:qk-layer}
\end{equation}
for $0 \le \ell \le L$, where $\ca_\ell$ is defined as in~\eq{CA}. 
% Because of linearity, projection $W_\ell$ is the same as a value projection.

Image features $F_0, \dots, F_L$ do not change by injecting our \Ours into network $f$. However, the final global image representation and hence the prediction do change. In particular, at the last stage $L$, $\vq_{L+1}$ is used as a global image representation for classification, replacing \gap over $F_L$. The final prediction is $g(\vq_{L+1}) \in \real^C$. Unlike \gap, the weights of different image patches in the linear combination are non-uniform, enhancing the contribution of relevant patches in the prediction.

%------------------------------------------------------------------------------
%------------------------------------------------------------------------------
\input{tex/mainfig}
%------------------------------------------------------------------------------


\paragraph{Training}

In this sense, the network $f$ is pretrained and remains frozen while we learn the parameters of our \Ours on the same training set as one used to train $f$. The classifier is kept frozen too. Referring to~\eq{f-decomp}, $f_0, \dots, f_L$ and $g$ are fixed, while \gap is replaced by learned weighted averaging, with the weights obtained by the \Ours.

\paragraph{Inference}

As it stands, \Ours is not an interpretability method, but rather a modification of the baseline architecture, \ie, an attention-based pooling mechanism that replaces \gap to enhance the contribution of relevant image regions in the prediction. We are interested in investigating the interpretability properties of this modification. We therefore employ existing post-hoc, CAM-based interpretability methods to generate saliency maps with both baseline \gap and \Ours. We then compare interpretability metrics as well as classification accuracy.



==> WACV_Backups/tex_wacv/plots-ext.tex <==
%------------------------------------------------------------------------------
% hack for CVPR/ICCV style
\makeatletter
\@namedef{ver@everyshi.sty}{}
\makeatother

%------------------------------------------------------------------------------
% main packages
\usepackage[dvipsnames,svgnames,x11names]{xcolor}
\usepackage{tikzextern}
\usepackage{pgffor}

%------------------------------------------------------------------------------
% externalization
\newcommand{\extfig}[2]{\tikzsetnextfilename{fig/extern/#1}{#2}}
\newcommand{\noextfig}[1]{!!!}
\newcommand{\extdata}[1]{}


==> WACV_Backups/tex_wacv/plots-none.tex <==
\newcommand{\extfig}[2]{!!!}
\newcommand{\noextfig}[1]{!!!}
\newcommand{\extdata}[1]{}


==> WACV_Backups/tex_wacv/plots.tex <==
%------------------------------------------------------------------------------
% hack for CVPR/ICCV style
\makeatletter
\@namedef{ver@everyshi.sty}{}
\makeatother

%------------------------------------------------------------------------------
% main packages
\usepackage[dvipsnames,svgnames,x11names]{xcolor}
\usepackage{tikz}
\usetikzlibrary{arrows.meta,shapes,calc,matrix,fit,positioning,backgrounds,decorations.markings,fadings}
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\pgfplotsset{compat=1.9}
\usepackage{xstring}

%------------------------------------------------------------------------------
% externalization: requires defining \finalcopy first

\usepgfplotslibrary{external}
% \tikzexternalize[prefix=fig/extern/]
\newcommand{\extfig}[2]{\tikzsetnextfilename{#1}{#2}}
\newcommand{\noextfig}[1]{\tikzset{external/export next={false}}{#1}}
\newcommand{\extdata}[1]{\input{#1}}
\IfBeginWith*{\jobname}{fig/extern/}{\finalcopy}{}

%-----------------------------------------------------------------------------
% tikz styles

\tikzstyle{every picture}+=[
	remember picture,
	every text node part/.style={align=center},
	every matrix/.append style={ampersand replacement=\&},
]
\tikzstyle{tight} = [inner sep=0pt,outer sep=0pt]
\tikzstyle{node}  = [draw,circle,tight,minimum size=12pt,anchor=center]
\tikzstyle{op}    = [draw,circle,tight]
\tikzstyle{dot}   = [fill,draw,circle,inner sep=1pt,outer sep=0]
\tikzstyle{pt}    = [fill,draw,circle,inner sep=1.5pt,outer sep=.2pt]
\tikzstyle{box}   = [draw,rectangle,inner sep=3pt]
\tikzstyle{high}  = [black!60]
\tikzstyle{group} = [high,box,opacity=.5]
\tikzstyle{dim1}  = [fill opacity=.3,text opacity=1]
\tikzstyle{dim2}  = [fill opacity=.5,text opacity=1]
\tikzstyle{dim3}  = [fill opacity=.7,text opacity=1]
\tikzstyle{rectc} = [tight,transform shape]
\tikzstyle{rect}  = [rectc,anchor=south west]

%-----------------------------------------------------------------------------
% framed figures

\newcommand{\framed}[3][1]{\extfig{#2}{\tikz{
	\node[tight](a){\fig[#1]{#3}};
	\node[tight,draw=gray,fit=(a)]{};
}}}

%-----------------------------------------------------------------------------
% pgfplots general options

\newcommand{\leg}[1]{\addlegendentry{#1}}

\tikzset{every mark/.append style={solid}}
\pgfplotsset{%smooth,
	grid=both, width=\columnwidth, try min ticks=5,
	every axis/.append style={font=\small},
	every axis plot/.append style={thick,mark=none,mark size=1.8,tension=0.18},
	legend cell align=left, legend style={fill opacity=0.8},
	xticklabel={\pgfmathprintnumber[assume math mode=true]{\tick}},
	yticklabel={\pgfmathprintnumber[assume math mode=true]{\tick}},
	nodes near coords math/.style={
		nodes near coords={\pgfmathprintnumber[assume math mode=true]{\pgfplotspointmeta}},
	},
}

\pgfplotsset{
	dash/.style={mark=o,dashed,opacity=0.6},
	dott/.style={mark=o,dotted,opacity=0.6},
	nolim/.style={enlargelimits=false},
	plain/.style={every axis plot/.append style={},nolim,grid=none},
}
\newcommand{\kilo}[1]{\thisrow{#1}/1000}

%--------------------------------------------------------------------

% layers
\pgfdeclarelayer{bg4}
\pgfdeclarelayer{bg3}
\pgfdeclarelayer{bg2}
\pgfdeclarelayer{bg1}
\pgfdeclarelayer{fg1}
\pgfdeclarelayer{fg2}
\pgfdeclarelayer{fg3}
\pgfdeclarelayer{fg4}
\pgfsetlayers{bg4,bg3,bg2,bg1,main,fg1,fg2,fg3,fg4}

%------------------------------------------------------------------------------
% 3d drawing

\pgfkeys{/tikz/.cd, aspect/.store in=\aspect, aspect=1}
\pgfkeys{/tikz/.cd, depth/.store in=\depth, depth=.5}
\pgfkeys{/tikz/.cd, stepx/.store in=\step, stepx=1}

\tikzstyle{geom} = [line join=bevel,aspect=1,depth=.5,z={(\depth*\aspect,\depth)}]
\tikzstyle{wire} = [geom,draw,thick]

% 3d coordinates
\def\cx[#1,#2,#3]{#1}
\def\cy[#1,#2,#3]{#2}
\def\cz[#1,#2,#3]{#3}
\def\ex[#1,#2,#3]{#1,0,0}
\def\ey[#1,#2,#3]{0,#2,0}
\def\ez[#1,#2,#3]{0,0,#3}

% lines along x, y, or z
\newcommand{\zline}[3][]{%
\path[geom,#1] #2 -- +(\cx[#3],\cy[#3]);
}
\newcommand{\yline}[3][]{%
\path[geom,#1,shift={#2},xslant=\aspect]
	(0,0) -- +(\cx[#3],\depth*\cz[#3]);
}
\newcommand{\xline}[3][]{%
\path[geom,#1,shift={#2},yslant=1/\aspect]
	(0,0) -- +(\aspect*\depth*\cz[#3],\cy[#3]);
}

% rectangles / grids along x, y, or z
\newcommand{\zrect}[3][]{%
\path[geom,#1] #2 rectangle +(\cx[#3],\cy[#3]);
}
\newcommand{\yrect}[3][]{%
\path[geom,#1,shift={#2},xslant=\aspect]
	(0,0) rectangle +(\cx[#3],\depth*\cz[#3]);
}
\newcommand{\xrect}[3][]{%
\path[geom,#1,shift={#2},yslant=1/\aspect]
	(0,0) rectangle +(\aspect*\depth*\cz[#3],\cy[#3]);
}
\newcommand{\xgrid}[3][]{%
\path[geom,#1,shift={#2},yslant=1/\aspect,xstep=\aspect*\depth*\step]
	(0,0) grid +(\aspect*\depth*\cz[#3],\cy[#3]);
}

% parallepiped
\newcommand{\para}[4][]{%
\zrect[#1]{(#3)}{#4}                 % front
\yrect[#1]{($(#3)+(\ey[#4])$)}{#4}   % top
\xrect[#1]{($(#3)+(\ex[#4])$)}{#4}   % right
\path[geom]
	(#3) coordinate(#2-southwest)
	($(#3)+(#4)$) coordinate(#2-northeast)
	($(#3)+(\ey[#4])$) coordinate(#2-northwest)
	($(#3)+(#4)-(\ey[#4])$) coordinate(#2-southeast)
	($(#3)+.5*(\ex[#4])$) coordinate(#2-south)
	($(#3)+(#4)-.5*(\ex[#4])$) coordinate(#2-north)
	($(#3)+.5*(\ex[#4])+.5*(#4)$) coordinate(#2-center)
	(#2-southwest |- #2-center) coordinate(#2-west)
	(#2-center -| #2-northeast) coordinate(#2-east)
	;
}


==> WACV_Backups/tex_wacv/related.tex <==
\section{Related Work}

\subsection{Interpretability}

To open up the black-box behavior of deep neural networks, model interpretability is mainly investigated along two directions~\citep{lipton18, guidotti2018survey, zhang2021survey}:
\begin{enumerate}[itemsep=2pt, parsep=0pt, topsep=3pt]
	\item \emph{Post-hoc interpretability} considers the model as a black-box and provides explanations based on inputs and outputs, without modifying the model or its training process.
	\item \emph{Transparency} modifies the model or the training process to better explain the behavior of the inner parts of the model.
\end{enumerate}

\paragraph{Post-hoc interpretability}
Approaches can be grouped into a number of possibly overlapping categories. \emph{Gradient-based methods}~\citep{adebayo2018local, springenberg2014striving, baehrens2010explain, simonyan2013deep, smilkov2017smoothgrad, bach2015pixel, sundararajan2017axiomatic} use the gradient of a target class score with respect to the input to compute the contribution of different input regions to the prediction. \emph{CAM-based methods}~\citep{DBLP:journals/corr/abs-1910-01279, DBLP:journals/corr/abs-1710-11063, DBLP:journals/corr/SelvarajuDVCPB16, fu2020axiom, jiang2021layercam, ramaswamy2020ablation} compute saliency maps as a linear combination of feature maps, with different definitions for the weights. \emph{Occlusion or masking-based methods}~\citep{petsiuk2018rise, fong2017interpretable, fong2019understanding, schulz2020restricting, ribeiro2016should} apply a number of candidate masks in the input space, measure their effect on the prediction and then combine them into a saliency map. Masking in feature space has been explored too~\cite{schulz2020restricting}. Finally, \emph{learning-based methods}~\citep{chang2018explaining, dabkowski2017real, phang2020investigating, zolna2020classifier, schulz2020restricting} learn an additional network or branch on extra data to produce an explanation map for a given input. 

Our method shares similarities with learning-based methods. In particular, we train an additional branch on the same training data as the network we aim to explain, but we only use the standard classification loss and we do not provide any explanation as output. Our method is also similar to CAM-based and masking-based methods exactly because we show that attention-based pooling is the same as masking in the feature space with weights obtained by a CAM-based saliency map.

\paragraph{Transparency}
Approaches are grouped in a number of categories according to the type of the given explanation. \emph{Rule-based methods}~\citep{wu2018beyond, wu2020regional} train a decision tree as a surrogate regularization term to force a network to be easily approximated by a decision tree.
% or learn a set of logit rules as an explanation~\citep{azzolin2022global}.
\emph{Hidden semantics-based methods}~\citep{bau2017network, zhou2018interpreting, zhang2018interpretable, zhou2014object} aim to make a convolutional network learn disentangled hidden semantics with hierarchical structure or object-level concepts.
\emph{Prototype-based methods}~\citep{li2018deep, chen2019looks} learn a set of prototypes or parts as an intermediate representation in the network, which can be aligned with categories. \emph{Attribution-based methods}~\citep{ismail2021improving, Zhou_2022_BMVC, ross2017right, ghaeini2019saliency} usually modify the architecture of a network or the training process to help post-hoc methods produce better saliency maps. Unlike~\citep{ross2017right, ghaeini2019saliency}, saliency guided localization~\citep{Zhou_2022_BMVC} does not need ground truth explanations but replaces them with information bottleneck attribution~\citep{schulz2020restricting}. Finally, saliency-guided training~\citep{ismail2021improving} minimizes the KL divergence between the output of original and masked images.

Our method belongs to attribution-based methods. We introduce a learnable cross-attention stream into the network as a pooling mechanism to replace \gap. As a result, post-hoc attribution-based methods can provide a better explanation. Although the network is modified, the training process is not: the network and classifier are pretrained and kept frozen while we learn the paramaters of our stream.

%------------------------------------------------------------------------------

\subsection{Attention-based architectures}

Attention is a powerful mechanism that has been introduced into convolutional networks in several ocaasions~\citep{bello2019attention, ramachandran2019stand, shen2020global}. With the success of vision transformers (ViT)~\citep{dosovitskiy2020image}, fully attention-based architectures are now competitive with convolutional networks. To benefit from both self-attention and convolutional layers, some hybrid architectures employ convolutional layers before the vision transformer~\citep{graham2021levit,xiao2021early}. Others, such as Swin~\citep{liu2021swin} and PiT~\citep{heo2021rethinking}, introduce a pyramid structure to share local spatial information while reducing the spatial resolution, as in convolutional networks. 

Conformer~\citep{peng2021conformer} proposes a dual network structure to retrain and fuse local convolutional features with global representations. Our method merely provides a simple attention-based pooling mechanism inspired by transformers that can work with any architecture, even pretrained and frozen. SCOUTER~\citep{li2021scouter} uses slot attention~\cite{locatello2020object} to build a class specific pooling mechanism, which does not scale well to more than 20 classes. Our mechanism is based standard cross attention, it is class agnostic and scales up to 1000 classes, improving post-hoc interpretability without degrading classification accuracy. PatchConvNet~\citep{touvron2021augmenting} replaces global average pooling by an attention-based pooling layer. Our method is similar in this respect, but uses information collected from the entire network by a parallel processing stream. We introduce our mechanism into any convolutional network and study its effect on post-hoc interpretability.









==> fig/tex/fig_connection_cr.tex <==
\begin{figure}[H]
    \centering
    % editable at https://docs.google.com/drawings/d/1nfqVV_dNqSV9g5UBuNopPLvubcEZx-vvg4K0ZCvNdfU/edit
    %\fig[.7]{CA-CAM}
    \includegraphics[width=.475\textwidth]{fig/CA-CAM.pdf}
    %\vspace{1.5pt}
    \caption{\textbf{Visualization of eq.(\red{5})).} On the left, a feature tensor $\vF \in \real^{w \times h \times d}$ is multiplied by the vector $\valpha \in \real^d$ in the channel dimension, like in $1 \times 1$ convolution, where $w \times h$ is the spatial resolution and $d$ is the number of channels. This is \emph{cross attention} (CA) \cite{dosovitskiy2020image} between the query $\valpha$ and the key $\vF$. On the right, a linear combination of feature maps $F^1, \dots, F^d \in \real^{w \times h}$ is taken with weights $\alpha_1, \dots, \alpha_d$. This is a \emph{class activation mapping} (CAM) \cite{zhou2016learning} with class agnostic weights. Eq.(\red{5})expresses the fact that these two quantities are the same, provided that $\valpha = (\alpha_1, \dots, \alpha_d)$ and $\vF$ is reshaped as $F = (\vf^1 \dots \vf^d) \in \real^{p \times d}$, where $p = wh$ and $\vf^k = \vect(F^k) \in \real^{p}$ is the vectorized feature map of channel $k$.}
    \label{fig:connection}
    
\end{figure}

==> fig/tex/figure_ra-passes.tex <==
\begin{figure*}[ht]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{cccccccc}
           \mr{2}{}&\mr{2}{\Th{Original}}&\mc{3}{\Th{First Pass}}&\mc{3}{\Th{Second Pass}}\\
            & &\gap-\Th{GC} & \ours-\Th{GC} & \ours-\Th{RA} &\gap-\Th{GC} & \ours-\Th{GC} & \ours-\Th{RA}\\
           {\rotatebox{90}{\small text}}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/Original/1019.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/F-Base-CAM/1019.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/F-Stream-CAM/1019.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/F-Stream-Raw/1019.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/S-Base-CAM/1019.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/S-Stream-CAM/1019.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/S-Stream-Raw/1019.jpeg}\\

           {\rotatebox{90}{\small text}}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/Original/274.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/F-Base-CAM/274.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/F-Stream-CAM/274.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/F-Stream-Raw/274.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/S-Base-CAM/274.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/S-Stream-CAM/274.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/S-Stream-Raw/274.jpeg}\\

           {\rotatebox{90}{\small text}}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/Original/963.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/F-Base-CAM/963.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/F-Stream-CAM/963.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/F-Stream-Raw/963.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/S-Base-CAM/963.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/S-Stream-CAM/963.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/S-Stream-Raw/963.jpeg}\\

           {\rotatebox{90}{\small text}}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/Original/1944.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/F-Base-CAM/1944.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/F-Stream-CAM/1944.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/F-Stream-Raw/1944.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/S-Base-CAM/1944.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/S-Stream-CAM/1944.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/S-Stream-Raw/1944.jpeg}\\         

          {\rotatebox{90}{\small text}}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/Original/711.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/F-Base-CAM/711.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/F-Stream-CAM/711.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/F-Stream-Raw/711.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/S-Base-CAM/711.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/S-Stream-CAM/711.jpeg}&\includegraphics[width=0.1\textwidth]{Images/CLS_Passes/S-Stream-Raw/711.jpeg}\\          
    \end{tabular}
    }
    \caption{\emph{Comparison between }}
    \label{fig:com_forwards}
\end{figure*}

==> tab/tab_comparison_correct.tex <==
\begin{table}[H]
    \centering
    \scriptsize
    \setlength{\tabcolsep}{1.5pt}
    \begin{tabular}{cccccccc}\toprule
        \Th{Network}&\Th{Pooling}&\Th{Acc}$\uparrow$&P($y^c$)$\uparrow$&P($\hat{y}$)$\uparrow$&P$(y^c)_{\tiny\checkmark} \uparrow$&P$(y^c)_\times\uparrow$&P$(\hat{y})_\times\downarrow$\\
         \mr{2}{\Th{ResNet-50}}&\gap&74.55&67.68&78.41&87.06&\textbf{10.93}&\textbf{53.09}\\
         &\ours&\textbf{74.70}&\textbf{69.39}&\textbf{81.42}&\textbf{89.31}&10.66&58.17\\\midrule
         \mr{2}{\Th{ConvNeXt-B}}&\gap&\textbf{83.72}&57.47&63.36&66.87&9.12&\textbf{45.31}\\
         &\ours&83.51&\textbf{81.21}&\textbf{91.10}&\textbf{95.13}&\textbf{10.66}&70.66\\\bottomrule
    \end{tabular}
    \caption{\emph{Predictive power per representation}}
    \label{tab:predpower}
\end{table}



==> tab/tab_gt_v_pred_older.tex <==
\begin{table*}[t]
    \centering
    \footnotesize
    \setlength{\tabcolsep}{2.5pt}
    \renewcommand{\arraystretch}{1.15}
    \begin{tabular}{llcccccc|cccccc}
        \cline{4-13}
        &&&\multicolumn{5}{c|}{\Th{Groundtruth Labels}}&\mc{5}{\Th{Predicted Labels}}\\\hline
        \Th{Network}&\Th{Attribution}&\Th{Pooling}&\Th{AD$\downarrow$}&\Th{AG$\uparrow$}&\Th{AI$\uparrow$}&\Th{I$\uparrow$}&\Th{D$\downarrow$}&\Th{AD$\downarrow$}&\Th{AG$\uparrow$}&\Th{AI$\uparrow$}&\Th{I$\uparrow$}&\Th{D$\downarrow$}\\\hline
        \mr{7}{\Th{ResNet50}}&\mr{2}{Grad-CAM}&\gap&13.01&17.58&44.51&65.19&\textbf{11.26}&14.86&18.56&38.77&74.00&\textbf{12.31}\\
        &&\ours&\textbf{12.52}&\textbf{22.68}&\textbf{48.62}&\textbf{67.68}&11.50&\textbf{13.73}&\textbf{24.11}&\textbf{43.63}&\textbf{77.13}&12.58\\\cline{2-13}
        &\mr{2}{Grad-CAM++}&\gap&\textbf{13.62}&16.21&44.50&64.59&\textbf{11.50}&15.06&17.31&37.45&73.28&\textbf{12.58}\\
        &&\ours&13.75&\textbf{19.68}&\textbf{45.21}&\textbf{66.65}&12.05&\textbf{14.05}&\textbf{21.34}&\textbf{41.27}&\textbf{76.01}&13.17\\\cline{2-13}
        &\mr{2}{Score-CAM}&\gap&8.83&17.97&48.46&64.85&\textbf{11.86}&Check&Check&Check&Check&Check\\
        &&\ours&\textbf{7.09}&\textbf{23.65}&\textbf{54.20}&\textbf{67.56}&11.93&Check&Check&Check&Check&Check\\\hline
        \mr{7}{\Th{ConvNeXt-B}}&\mr{2}{Grad-CAM}&\gap&35.52&2.59&15.88&48.98&\textbf{26.95}&35.79&2.17&10.32&53.26&\textbf{28.72}\\
        &&\ours&\textbf{18.53}&\textbf{13.88}&\textbf{32.23}&\textbf{80.39}&39.85&\textbf{20.43}&\textbf{14.00}&\textbf{27.85}&\textbf{88.26}&42.59\\\cline{2-13}
        &\mr{2}{Grad-CAM++}&\gap&42.29&2.73&15.45&48.85&\textbf{28.97}&TBA&TBA&TBA&TBA&TBA\\
        &&\ours&\textbf{20.51}&\textbf{11.49}&\textbf{28.76}&\textbf{79.93}&41.94&21.56&11.91&24.74&87.78&44.21\\\cline{2-13}
        &\mr{2}{Score-CAM}&\gap&43.55&2.23&15.67&Check&Check&TBA&TBA&TBA&TBA&TBA\\
        &&\ours&23.51&11.04&27.35&Check&Check&TBA&TBA&TBA&TBA&TBA\\\hline
    \end{tabular}
    \caption{\emph{Comparison of Interpretability metrics between \Ours vs \gap }}
    \label{tab:intrecon-all}
\end{table*}

==> tex/exp_ablation.tex <==
\subsection{Ablation}
\label{sec:gen_ablation}

We conduct ablation experiments on ResNet50 because of its modularity and ease of modification. We investigate the effect of the cross-attention block design and the placement of the \Ours relative to the backbone network.
The appendix further includes experiments on class-agnostic \vs class-specific representations.

%------------------------------------------------------------------------------

\paragraph{Cross-attention block design}

Following transformers~\cite{NIPS2017_3f5ee243,dosovitskiy2020image}, it is possible to add more layers in the cross-attention block. We consider a variant referred to as \PO, which uses linear projections $W_\ell^K, W_\ell^V \in \real^{d_\ell \times d_\ell}$ on the key and value
\begin{equation}
	\ca_\ell(\vq_\ell, F_\ell) \defn (F_\ell W^V_\ell)\tran h_\ell(F_\ell W^K_\ell \vq_\ell)\in \real^{d_\ell},
\label{eq:proj_ca}
\end{equation}
while equation~\eq{qk-layer} remains.

We consider two variants. One, referred to as \PO, uses linear projections $W_\ell^K, W_\ell^V \in \real^{d_\ell \times d_\ell}$ on the key and value
\begin{equation}
	\ca_\ell(\vq_\ell, F_\ell) \defn (F_\ell W^V_\ell)\tran h_\ell(F_\ell W^K_\ell \vq_\ell)\in \real^{d_\ell}.
\label{eq:proj_ca}
\end{equation}
In another variant, referred to as \OM, an MLP follows each cross attention block, defined as
\begin{equation}
	\mlp_\ell(\vq_\ell) = W_\ell^2 \gelu(W_\ell^1 \vq_\ell + b_\ell^1) + b_\ell^2,
\label{eq:mlp_ca}
\end{equation}
where $W_\ell^1 \in \real^{2d_\ell \times d_\ell}$ and $W_\ell^1 \in \real^{d_\ell \times 2d_\ell}$. In both cases, equation~\eq{qk-layer} remains. The combination of the two variants is referred to as \POM.

We compare the effect on accuracy when adding one of the variants to the backbone (just after the last residual block). \autoref{tab:CA_variations} demonstrates this assessment.

%------------------------------------------------------------------------------
\begin{table}
\centering
%\resizebox{\columnwidth}{!}{%
\scriptsize
\begin{tabular}{lcc}\\\toprule
	\Th{Block Type}&\Th{$\#$Params}&\Th{Acc}\\\midrule
	CA&4.20M&74.63\\
	Proj$\rightarrow$CA&12.58M&74.19\\
	CA$\rightarrow$MLP&20.97M&-\\
	Proj$\rightarrow$CA$\rightarrow$MLP&29.36M&-\\\bottomrule
\end{tabular}
%}
\vspace{3pt}
\caption{Comparison of classification performance when one cross attention block is added into the last residual block of ResNet-50.}
\label{tab:CA_variations}
\end{table}
%------------------------------------------------------------------------------

We observe that the introduction of the basic design of the cross attention module outperforms the classification properties of that which uses projection of the input features to compute the subsequent representation. We hypothesize that maintaining the features without any projection allows the [class] token to better collect global information, as patch information is maintained in the same space that the already trained classifier relies on to perform classification.
On another hand, we also note that the introduction of an MLP to update said representation is not feasible given instability during training, for this reason we decide not to pursue further experimentation with this idea.

%------------------------------------------------------------------------------
\begin{table}
\centering
\scriptsize
%\resizebox{\columnwidth}{!}{%}
\begin{tabular}{lcc}\toprule
	\Th{Block Type}&\Th{$\#$Params}&\Th{Accuracy}\\\midrule
	\our&6.96M&74.70\\
	\PO&18.13M&74.41\\\bottomrule
\end{tabular}
%}
%\vspace{3pt}
\caption{\emph{Different cross-attention block design for \Ours.} Classification accuracy and parameters using ResNet-50 on ImageNet. \Th{$\#$Param}: parameters of \Ours only.}
\label{tab:dif_streams}
\end{table}
%------------------------------------------------------------------------------

Results are reported in \autoref{tab:dif_streams}. We observe that the stream made of vanilla CA blocks~\eq{CA} offers slightly better accuracy than projections~\eq{proj_ca}, while having less parameters. We also note that most of the computation takes place in the last residual stages, where the channel dimension is the largest. To keep our design simple, we choose the vanilla solution without projections~\eq{CA} by default.

%------------------------------------------------------------------------------

\paragraph{\Ours placement}
\label{ab:placement}

To validate the design of \Ours, we measure the effect of its depth on its performance \vs the baseline \gap in terms of both classification accuracy / number of parameters and classification metrics for interpretability. In particular, we place the stream in parallel to the network $f$, starting at stage $\ell$ and running through stage $L$, the last stage of $f$, where $0 \le \ell \le L$. Results are reported in \autoref{tab:intrecog-resnet}.

%------------------------------------------------------------------------------
\begin{table}
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
%\resizebox{\columnwidth}{!}{%}
\begin{tabular}{lcccccc}\toprule
	\mc{7}{\Th{Accuracy and Parameters}}\\\midrule
	&\Th{Placement}&\mc{2}{\Th{CLS dim}}&\mc{2}{\Th{\#Param}}&\Th{Acc$\uparrow$}\\\midrule

	&$S_0-S_4$&\mc{2}{$64$}  &\mc{2}{6.96M}&\textbf{74.70}\\  % 6.963.264
	&$S_1-S_4$&\mc{2}{$256$} &\mc{2}{6.95M}&74.67\\           % 6.947.072
	&$S_2-S_4$&\mc{2}{$512$} &\mc{2}{6.82M}&74.67\\           % 6.816.256
	&$S_3-S_4$&\mc{2}{$1024$}&\mc{2}{6.29M}&74.67\\           % 6.292.480
	&$S_4-S_4$&\mc{2}{$2048$}&\mc{2}{4.20M}&74.63\\\midrule   % 4.196.352

	\mc{7}{\Th{Interpretability Metrics}}\\\midrule
	\Th{Method}&\Th{Placement}&\Th{AD$\downarrow$}&\Th{AG$\uparrow$}&\Th{AI$\uparrow$}&\Th{I$\uparrow$}&\Th{D$\downarrow$}\\\midrule

	\mr{5}{\Th{Grad-CAM}}&$S_0-S_4$&\textbf{12.54}&\textbf{22.67}&48.56&75.53&13.50\\ % Checked
		&$S_1-S_4$&12.69&22.65&48.31&75.53&13.41\\ % Checked
		&$S_2-S_4$&\textbf{12.54}&21.67&\textbf{48.58}&75.54&13.50\\ % Running
		&$S_3-S_4$&12.69&22.28&47.89&\textbf{75.55}&13.40\\ % Running
		&$S_4-S_4$&12.77&20.65&47.14&74.32&\textbf{13.37}\\\midrule % Checked

	\mr{5}{\Th{Grad-CAM++}}&$S_0-S_4$&13.99&19.29&44.60&75.21&13.78\\ % Checked
		&$S_1-S_4$&13.99&19.29&44.62&75.21&13.78\\ % Checked
		&$S_2-S_4$&13.71&\textbf{19.90}&\textbf{45.43}&75.34&13.50\\ % Running
		&$S_3-S_4$&13.69&19.61&45.04&\textbf{75.36}&13.50\\ % Running
		&$S_4-S_4$&\textbf{13.67}&18.36&44.40&74.19&\textbf{13.30}\\\midrule % Checked

	\mr{5}{\Th{Score-CAM}}&$S_0-S_4$&\textbf{7.09}&23.65&54.20&74.91&14.68\\ % Checked
		&$S_1-S_4$&\textbf{7.09}&23.65&54.20&74.92&14.68\\ % Checked
		&$S_2-S_4$&\textbf{7.09}&\textbf{23.66}&\textbf{54.21}&74.91&14.68\\ % Running
		&$S_3-S_4$&7.74&23.03&52.92&\textbf{74.97}&14.65\\ % Running
		&$S_4-S_4$&7.52&19.45&50.45&74.19&\textbf{14.46}\\\bottomrule % Checked
\end{tabular}
% }
%\vspace{3pt}
\caption{\emph{Effect of stream placement} on accuracy, parameters and interpretability metrics  for ResNet-50 on ImageNet. $S_\ell-S_L$: \Ours runs from stage $\ell$ to $L$ (last); \Th{$\#$Param}: parameters of \Ours only.}
\label{tab:intrecog-resnet}
\end{table}
%------------------------------------------------------------------------------

From the interpretability metrics as well as accuracy, we observe that stream configurations that allow for iterative interaction with the network features obtain the best performance, although the effect of stream placement is small in general. In many cases, the lightest stream of only one cross attention block ($S_4-S_4$) is inferior to options allowing for more interaction.
Since starting the stream at early stages has little effect on the number of parameters and performance is stable, we choose to start the stream in the first stage ($S_0-S_4$) by default.

%------------------------------------------------------------------------------



%------------------------------------------------------------------------------

%% Top design, bottom interp metrics
%% More parts for experiments

% Ablation of histogram of diferences with extreme cases


==> tex/exp_var.tex <==
\subsection{Variations}
\label{subsec:variations}

As in \cite{dosovitskiy2020image}, we observe that it is possible to modify the cross attention mechanism to further update features after the linear projection following attention computation. Moreover, it is also possible to project the input features to the space in which the [class] token lies within. We define the following variations:

\paragraph{Cross Attention with MLP}
The work of \cite{NIPS2017_3f5ee243} and \cite{dosovitskiy2020image} introduce a MLP or feedforward network to capture and process local patterns more globally. Thus we propose to add a MLP on top of Cross Attention, as Vision transformers:
% Regarding the architecture of transformers, we observe that following attention operation and the following projection, a feedforward network or MLP is used to further update the representation produced. To this end, we consider:
\begin{equation}
    \mbox{MLP}_\ell(\vq_{\ell}) = \mbox{GELU}(\vq_\ell W_{in}+b_{in})W_{out}+b_{out}.
    % \vq_{\ell+1} = W_\ell \cdot \ca_\ell(\vq_\ell, F_\ell),
    \label{eq:mlp_ca}
\end{equation}
Where the input and output dimensions remain the same and the inner layer has reduced dimension of $d_{in} = d_l\times 2$.\\

\paragraph{Projected Cross Attention}
On the operational level, our Cross Attention Block leverages the interactions between the [CLS] token and the features of a given model for a given layer \textit{l}, projecting to the dimension at the following stage \textit{l+1}. It is however possible to preserve the space in which this token lies, by the projection of the features at a given layer to the dimension of [CLS]
\begin{equation}
    % \mbox{CA}_\ell(Q, F_{\ell}) = \mbox{softmax}(\frac{Q_{\ell}(F_{\ell}W^K)^\top}{\sqrt{d_Q}})F_{\ell}W^V
    \ca_\ell(\vq_\ell, F_\ell) \defn (F_\ell W^V_\ell)\tran h_\ell(F_\ell W^K_\ell \vq_\ell)\in \real^{d_\ell}.
    % \ca_\ell(\vq_\ell, F_\ell) \defn F_\ell\tran \va = F_\ell\tran h_\ell(F_\ell \vq_\ell) \in \real^{d_\ell}.
    \label{eq:proj_ca}
\end{equation}
Where the projections are parameter matrices $W^K, W^V \in \real^{d_\ell\times d_Q}$.

On \autoref{sec:gen_ablation} we experiment with the different proposals for the cross attention mechanism and its integration into the CLS-Stream.

==> tex/plots-ext.tex <==
%------------------------------------------------------------------------------
% hack for CVPR/ICCV style
\makeatletter
\@namedef{ver@everyshi.sty}{}
\makeatother

%------------------------------------------------------------------------------
% main packages
\usepackage[dvipsnames,svgnames,x11names]{xcolor}
\usepackage{tikzextern}
\usepackage{pgffor}

%------------------------------------------------------------------------------
% externalization
\newcommand{\extfig}[2]{\tikzsetnextfilename{fig/extern/#1}{#2}}
\newcommand{\noextfig}[1]{!!!}
\newcommand{\extdata}[1]{}


==> tex/plots-none.tex <==
\newcommand{\extfig}[2]{!!!}
\newcommand{\noextfig}[1]{!!!}
\newcommand{\extdata}[1]{}

